Semantic Parallelism: Redefining Efficient MoE Inference via Model-Data Co-Scheduling

Prevailing LLM serving engines employ expert parallelism (EP) to implement multi-device inference of massive MoE models. However, the efficiency of expert parallel inference is largely bounded by inter-device communication, as EP embraces expensive all-to-all collectives to route tokens to the remote experts if not collocating on the same GPU/NPU device. Nevertheless, state-of-the-art schemes treat expert device-placement and request (or token) device-scheduling as separate concerns, triggering excessive communication between them and compromising inference efficiency This paper proposes Semantic Parallelism, a novel parallelism paradigm that minimizes the steep communication costs in EP-centric MoE serving via model-data collaborative scheduling. We implement Semantic Parallelism in a framework called Sem-MoE. Sem-MoE maximally collocates experts and their activating tokens onto the same device using proactively modeled activation likelihood between them and introduces three key techniques: (1) Offline model scheduling, which preliminarily clusters and collocates experts onto devices based on their co-activation tendencies for certain classes of input. (2) Online inter-request data scheduling for Attention-DP setups, which proactively rebatches incoming requests onto the device that hosts experts most likely and frequently activated by the corresponding requests. (3) Online intra-request data scheduling for Attention-TP setups, which seamlessly fuses a token reshuffling procedure into the original inference pipeline and proactively reschedules tokens to devices to reduce dispersed remote routing. We build Sem-MoE into a prevailing LLM serving engine SGLANG. Experiments show our collaborative scheduling approach can effectively reduce the all-to-all communication volume in EP and achieve superior inference throughput compared to existing solutions.

==> expr-new.tex <==
\section{Experiment}\label{sec:expr}

\begin{table}[t]
    \centering
    % \resizebox{\linewidth}{!}{
    \begin{tabular}{l|l}
        \hline
        \textbf{Server} & \textbf{Configuration} \\  
        \hline
        GPU-Server-A  & \begin{tabular}[l]{@{}l@{}} CPU: Two 44-core Intel 8458P CPUs \\ 
        CPU RAM: 2TB DDR5\\GPU: 8 cards, GPU RAM: 96GB HBM per card \\Inter-GPU: 900GBps high-speed link \end{tabular}                                                                    \\
        \hline
        GPU-Server-B & \begin{tabular}[l]{@{}l@{}}CPU: Two 44-core Intel 8458P CPUs \\ CPU RAM: 1TB DDR5\\GPU: 8 cards, GPU RAM: 48GB GDDR6 per card  \\ Inter-GPU: 2*PCIe switch (64GBps), UPI (20GBps) \end{tabular} 
        \\
        \hline
    \end{tabular}
    % }
    \caption{Experiment hardware configuration}
    \vspace{-15pt}
    \label{table:envs}
\end{table}

% \subsection{Experimental Setup}\label{sec:expr:setting:env}
\subsection{Experimental Environments}\label{sec:expr:setting:env}
We evaluate Sem-MoE on two 8-GPU servers with different interconnect speeds and topologies (cf., Table~\ref{table:envs}). \textbf{(a) GPU-Server-A: fast homogeneous interconnects.} GPU-Server-A represents commodity GPU servers unified for both training and inference, which are configured with 96GB-HBM per GPU and fast homogeneous interconnects. GPUs inside a server can communicate with each other at a premium bandwidth (900GBps). 
\textbf{(b) GPU-Server-B: slow heterogeneous interconnects.} GPU-Server-A represents commodity GPU servers dedicated to economic inference, which have no HBM and no high-speed NVLink interconnects. Each server has eight GPUs (48GB GDDR6); the left group of four GPUs is interconnected via a PCIe-5.0 switch (63.01GBps) and the right group of four GPUs holds the same symmetric configuration. Any GPU in one group communicating with another GPU in the other group needs to pass through a slow indirect link, i.e., CPUs' UPI (Ultra Path Interconnect) interface (20.8GBps). 

\subsection{Models, Datasets and Workload Traces}\label{sec:expr:setting:model}

\textbf{Model.} We choose two types of typical MoE models for evaluation, i.e., MoE models with \textit{a large number of small experts}, represented by DeepSeek-V2, and MoE models with \textit{a small number of large experts}, represented by Mixtral-8x7B. Both DeepSeek-V2 and Mixtural-8x7B are prevailing open-sourced MoE models.
\iffalse
We use the following three representative datasets to evaluate \LTY. \textbf{LongBench}~\cite{longbenchdataset} is a bilingual, multi-task benchmark for comprehensive assessments of long context understanding capabilities of LLMs, which contains six major categories of tasks including document QA, summarization, few-shot learning, synthetic tasks, and code completion. \textbf{GSM8K} (Grade School Math 8K)~\cite{cobbe2021gsm8k} is a dataset that includes 8.5K high-quality, grade-school-level math problems. The dataset was created to support the task of question answering that requires multi-step reasoning. The \textbf{HumanEval}~\cite{humaneval} dataset includes 164 programming problems with function signature, docstring, body, and several unit tests.
\fi

\textbf{Dataset.} We use the following three representative datasets \textit{LongBench}~\cite{longbenchdataset}, \textit{GSM8K} (Grade School Math 8K)~\cite{cobbe2021gsm8k} and \textit{HumanEval}~\cite{humaneval}.
\textbf{Workload.} It is important that workload characteristics, especially the length of input (i.e., prefilling) and output (i.e., decoding) per user request, should reflect the characteristics of real requests in production settings. We draw real requests' input and output length from the Mooncake production trace~\cite{qin2024mooncakekvcachecentricdisaggregatedarchitecture} and the Azure LLM Inference Trace~\cite{stojkovic2024dynamollmdesigningllminference}.% 
%
\iffalse
\footnote{The MoonCake trace contains 23,608 chatting requests sampled over one hour within one production inference cloud at MoonCake. The Azure LLM inference Trace contains chatting and coding requests sampled from two LLM inference services in Azure and was collected on May 2024.}. %
%
\fi
To synthesize a request, we first randomly sample a pair of input and out length from the MoonCake or the Azure trace with equal probability, and secondly, sample an entry from LongBench, GSM8K, or HumanEval with equal probability to realize the entry's prefilling and decoding (up to the sampled length).


% \begin{table}
%     \centering
%     \resizebox{\linewidth}{!}{
%     \begin{tabular}{c|c|c}
%     \hline
%     \textbf{Configuration} & \textbf{Mixtral-8x7B} & \textbf{DeepSeek-V2} \\
%     \hline
%     \# total params & 47B & 236B \\
%     \hline
%     top-k & 2 & 6\\
%     \hline
%     number of layers & 32 & 60 \\
%     \hline
%     number of routed experts & 8 & 160 \\
%     \hline
%     number of shared experts & 0 & 2 \\
%     \hline
%     \end{tabular}
%     }
%     \caption{Experiment model configuration}
%     \label{table:model-config}
%     % \vspace{-15pt}
% \end{table}

\begin{figure*}[t]
    \centering
    \subfigure[DeepSeek-V2 on GPU-Server-A (TP8-EP8).]{
    \label{fig:ds-ltc2tpt-h20}
    \includegraphics[width=.45\linewidth]{figures/deepseek-h20.pdf}
    }
    \subfigure[Mixtral-8x7B on GPU-Server-A (TP8-EP4TP2).]{
    \label{fig:mx-ltc2tpt-h20}
    \includegraphics[width=.45\linewidth]{figures/mixtral-h20.pdf}
    }
    \subfigure[DeepSeek-V2 on GPU-Server-B (TP8-EP8).]{
    \label{fig:ds-ltc2tpt-l40s}
    \includegraphics[width=.45\linewidth]{figures/deepseek-l40s.pdf}
    }
    \subfigure[Mixtral-8x7B on GPU-Server-B (TP8-EP4TP2).]{
    \label{fig:mx-ltc2tpt-l40s}
    \includegraphics[width=.45\linewidth]{figures/mixtral-l40s.pdf}
    }
    \caption{Inference throughput under TTFT, TPOT and p90-TBT latency constraints. DS-MoE: DeepSpeed-MoE. s-MoE: Speculative MoE, s-TS: Speculative Token Shuffling, s-EG: Speculative Expert Grouping. Note we tune parallel configurations and report the one DeepSpeed-MoE performs best.}
    % \vspace{-0.5cm}
    \label{fig:ltc2tpt}
\end{figure*}

\subsection{Baselines and Performance Metrics}\label{sec:expr:baselines}

We build \LTY\ into two state-of-the-art MoE serving frameworks, each with differently implemented inference optimizations spanning parallelization schemes, high-performance fused kernels, quantization, etc.

\textbf{TP-EP Baseline - DeepSpeed-MoE, DeepSpeed-TED, and Tutel:} DeepSpeed-MoE \cite{pmlr-v162-rajbhandari22a} is a strong inference framework known for efficient scalable MoE computation and communication. DeepSpeed-TED \cite{deepspeed-ted} is an optimized version of DeepSpeed-MoE that further reduces communication overhead in DeepSpeed-MoE. Tutel~\cite{tutel} is a customized version of DeepSpeed-MoE that optimizes both MoE training and inference with high-performance fused kernels. We choose an integrated version of DeepSpeed-MoE that includes all optimizations from DeepSpeed-TED and Tutel, as a state-of-the-art baseline, the baseline adopts TP for attention layers and EP for expert layers.

\textbf{TP Baseline - SGLang:} SGLang \cite{zheng2024sglangefficientexecutionstructured} is a prevailing open-source LLM inference framework, adopting a bunch of optimization including but not limited to continuous batching, paged attention, flash attention, radix-attention, advanced quantization, etc. SGLang declares optimizations for MoE models with high-performance, fused triton kernels \cite{triton-kernels} to implement TP-based parallelization for both attention and expert layers. 

\textbf{Metrics:} \textbf{Throughput} is the number of tokens (tokens/s) that an inference system can process under a time limit. We report the average throughput over a batch of prompts under the following latency constraints. \textbf{TTFT (Time to First Token)} measures the duration between the request's arrival and the first token's generation time. \textbf{TPOT (Time per Output Token} is the average time to generate an output token in the decoding phase, i.e., the total decoding time of a request normalized by the number of tokens generated. \textbf{TBT (Time between Tokens)} is the latency of every subsequent token generated in the decoding phase. We report the 90th percentile of TBT (p90 TBT). Following prior work~\cite{wu2024fastdistributedinferenceserving, wu2024loongserveefficientlyservinglongcontext}, we set the latency SLO as 5$\times$ of the latency (i.e., TTFT, TPOT, or p90 TBT) under the lightest input load (minimal input length times batch size sampled from datasets and trace). For each dataset, we use 20\% of the data to train the token activation prediction model, and the left 80\% is used to sample experimental requests.

\subsection{Evaluation - Speculative MoE vs. DeepSpeed-MoE}\label{sec:expr:e2e}

Figure~\ref{fig:ltc2tpt} shows the end-to-end performance evaluation of Speculative MoE (\LTY) and Deepspeed-MoE (DS-MoE). We evaluate two versions of \LTY,  namely \LTY~w/t s-TS, and \LTY~w/t s-TS+s-EG, to separate the contributions of Speculative Token shuffling (s-TS) and Speculative Expert Pre-grouping (s-EG), respectively.

\textbf{DeepSeek-V2.} For DeepSeek-V2, \LTY\ achieves 1.72x, 1.15x and 1.49x throughput improvements compared to DS-MoE on GPU-Server-A under TTFT, TPOT and p-90-TBT SLO constraints, respectively. Results show \LTY~outperforms DS-MoE even on the fastest (900GBps) homogeneous interconnects. Results show \LTY~ can still benefit production settings configured with high-end GPU interconnects (e.g., NVLink or UALink), as hardware and technology advances alone can not completely remove the current communication bottleneck of MoE inference. 





On GPU-Server-B, which is configured with slow heterogeneous interconnects (i.e., PCI-e and UPI), \LTY~ attains a much larger boost over
DS-MoE, where the throughput improvements rise to 1.89x, 2.35x, and 4.3x under the aforementioned SLOs. Results show that \LTY\ is more productive and supportive for economic inference settings that lack homogeneous high-speed hardware interconnects, and algorithm and software optimizations remain more effective and cost-efficient remedies. For DeepSeek-V2, separate analyses show that s-TS and s-EG on average contribute to $~$73\% and 27\% of the end-to-end throughput improvement of \LTY, respectively. The results validate the effectiveness and essentialness of the two key designs within \LTY.

\textbf{Mixtral-8x7B.} For Mixtral-8x7B, the throughput improvements of \LTY\ compared to DS-MoE is marginally lower to that of DeepSeek-V2, i.e.,  1.72x, 1.72xand 1.49x on GPU-Server-A and 2.34x, 2.70x and 2.92x on GPU-Server-B, under TTFT, TPOT and p90-TBT SLO constraints. The number of experts per layer of Mixtral-8x7B is smaller (only 8 experts per layer), and thus, the gated experts to route are more concentrated rather than dispersed, which results in lower effectiveness (only $~$4\% on average) for s-EG. However, s-TS remains effective in boosting DS-MoE. Overall, the consistent win of \LTY~ over DS-MoE on both DeepSeek-V2 featuring many small experts and Mixtral-8x7B featuring few big experts, and on both high-end and low-end interconnects substantiate \LTY~ as a generic approach to boost modern MoE inference.


\subsection{A Detailed Look at EP Communication Reduction}\label{sec:expr:breakdown}



In Figure~\ref{fig:single-layer-breakdown}, we show the LAR (Local Activation Rate) and the resulting latency of a single expert layer on GPU-Server-A. Local activation means the tokens' activation is routed to an expert collocated on the same GPU device, and thus remote routing and its associated EP communication can be skipped. A higher LAR is demanded. Results show, compared with DS-MoE, \LTY\ can increase LAR by 43\% and 61\% for DeepSeek-V2 and Mixtral-8x7B, which translates to 40.4\%/68.8\% latency reduction of the belonging expert layer. Besides DS-MoE and \LTY, other bars in the figure are measured by mocking the routing module of DS-MoE and skipping the delays in communication to fabricate hypothetical baselines just for reference. Note that a 100\% LAR may not be achieved in theory as different tokens can contradict each other to group their own hot experts but GPU memory is limited.


\subsection{Algorithm Evaluation}\label{sec:expr:algo}
The token and expert co-shuffling algorithm needs to find balanced co-clusters of tokens and experts, with experts having a maximal likelihood of being gated (routed) from tokens within the same cluster, and minimal likelihood across clusters. An additional regularizer is load balancing that ensures hot and cold experts are relatively evenly distributed. \LTY\ adopts a cross-entropy-optimization-based (CEO-based) algorithm to approximately solve the problem and is evaluated against two other baseline algorithms, METIS~\cite{karypis1997metis} and 2D Balanced KMeans, using the same predicted routing likelihood as affinity. METIS models the token-expert routing matrix as an undirected graph and solves the minimum k-cut solution. 2D Balanced KMeans performs a two-stage balanced KMeans clustering for tokens and experts with the predicted routing affinity separately. Figure~\ref{fig:algo_cmp} shows \LTY\ achieves the best LAR (highest communication reduction) with balanced expert clusters; its LAR and imbalance rate outperforms the best baseline by 14.2\% and 10.2\%, respectively. 

\begin{figure}[htbp]
    \centering
    \includegraphics[width=.9\linewidth]{figures/single-layer-l40s-breakdown.pdf}
    \caption{Local activation rate against overall EP overhead.}
    \label{fig:single-layer-breakdown}
    \vspace{-0.6cm}
\end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=.9\linewidth]{figures/algo_cmp_v2.pdf}
    \caption{Local activation rate ($\alpha$) and load-imbalance rate ($\beta$) of \LTY-CEO and baseline algorithms.}
    \label{fig:algo_cmp}
    \vspace{-0.3cm}
\end{figure}

% \subsection{Ablation Study}\label{sec:expr:ablation}


==> expr.tex <==
\section{Experiment}\label{sec:expr}

\begin{table}[t]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{c|c|c|c|c}
        \hline
        \textbf{Chip} & \textbf{Description} & \textbf{FP16 FLOPS} & \textbf{Intra-Node Bw.} & \textbf{Inter-Node Bw.} \\
        \hline
        L40S  & \begin{tabular}[c]{@{}c@{}}High Comp.\\ Low Comm.\end{tabular}    & 733T       & \begin{tabular}[c]{@{}c@{}}PCIe Gen4x16\\ 64GBps\end{tabular}    & /                                                                     \\
        \hline
        H20   &\begin{tabular}[c]{@{}c@{}}Low Comp.\\ High Comm.\end{tabular}    & 148T       & \begin{tabular}[c]{@{}c@{}}18-lane NVLink\\ 900GBps\end{tabular} & /                                                                     \\
        \hline
        H100  & \begin{tabular}[c]{@{}c@{}}High Comp.\\ Hybrid Comm.\end{tabular} & 1979T      & \begin{tabular}[c]{@{}c@{}}18-lane NVLink\\ 900GBps\end{tabular} & \begin{tabular}[c]{@{}c@{}}400GE CX7\\ 50GBps\end{tabular} 
                        \\
        \hline
    \end{tabular}
    }
    \caption{Experimental Environments}
    \vspace{-15pt}
    \label{table:envs}
\end{table}

% \subsection{Experimental Setup}\label{sec:expr:setting:env}
\subsection{Experimental Environments}\label{sec:expr:setting:env}
We carry out experiments on the following three types of real-world servers, representing different computation-communication characteristics. Table~\ref{table:envs} summarize the three types of servers.

% , including \textbf{L40S GPU server (single-node) with low interconnect bandwidth / high computing power}, \textbf{H20 GPU server (single-node) with high interconnect bandwidth/low computing power}, and \textbf{H100 GPU Server (Dual Node) with two dimensional network plane / high computing power}

\paragraph{L40S GPU server (single-node): low interconnect bandwidth, high computing power.} A server is equipped with 8 L40S cards, among which every 4 GPUs are governed by an Intel 8458P CPU and connected via a PCIe-5.0 switch (63.01GBps). Each GPU is equipped with 48GB GDDR6 memory. GPUs across PCIe switches inside a server can communicate through the Intel Ultra Path Interconnect (UPI) interface (20.8GBps). The L40S server is used to test the performance of \LTY\ in low-bandwidth single-node environments.

\paragraph{H20 GPU server (single-node): high interconnect bandwidth, low computing power.} A server is equipped with 8 H20 cards, among which every 4 GPUs are governed by an Intel 8458P CPU and a PCIe-5.0 switch. Each GPU is equipped with 96GB HBM3. GPUs inside a server are connected with 18-lane NVLINK-Gen4 (900GBps), which is much faster than traditional PCIe. However, the computation capacity of the H20 (148 TFLOPS for FP16) is much smaller than L40S (733 TFLOPS for FP16). Thus, the H20 server is adopted to evaluate the performance of \LTY\ in high-speed networks and low computation capacity environments.

\paragraph{H100 GPU Server (Dual Node): two dimensional network plane, high computing power.} The cluster contains 2 servers. Each server is equipped with 8 H100 cards, among which every 4 GPUs are governed by an Intel 8458P CPU and a PCIe-5.0 switch. Each GPU is equipped with 80GB HBM3e. GPUs inside a server are connected with 18-lane NVLINK-Gen3 (900GBps). In every PCIe switch, a 400GE dual-port ConnectX-7 network device is attached to enable inter-server communication. The H100 servers are used to test the scalability of \LTY\ in hybrid network environments.

\subsection{Models and Datasets}\label{sec:expr:setting:model}

Table~\ref{table:model-config} describes the configurations of the models used in the experiments. We choose two types of typical open-source MoE models for evaluatation. Models of the first category are MoE models with \textit{a large number of small experts}, represented by the DeepSeek series. The others are MoE models with \textit{a small number of large experts}, represented by the Mixtral family. The model uses the LongBench data set as the input for testing. We leverage the Mooncake production trace~\cite{qin2024mooncakekvcachecentricdisaggregatedarchitecture} to sampling inputs and outputs from the datasets. The mooncake trace is sampled from a subset of online request data of a 1-hour period. The trace dataset comprises 23,608 entries, with fields including timestamp, input\_length, output\_length, and KV cache block hash\_ids.

\begin{figure*}[t]
    \centering
    \includegraphics[width=.95\linewidth]{figures/single-node-e2e-latency-v2.pdf}
    \caption{\LTY\ vs baselines: latency and throughput on L40S/H20 servers. For DS-MoE, we select TP8 as the best configuration by comparing its performance under TP8/TP2EP4/TP4EP2/EP8.}
    \label{fig:ttft-e2e}
\end{figure*}

\begin{figure*}[t]
    \centering
    \includegraphics[width=.95\linewidth]{figures/multi-node-e2e-latency-v2.pdf}
    \caption{\LTY\ vs baselines: latency and throughput of DeepSeek-V2 on the 2-node 16*H100 cluster (As number of attention K/V heads of Mixtral-8x7B is 8, TP16 can not be adopted to deploy the model).}
    \label{fig:ttft-e2e-multi}
\end{figure*}

\begin{table}
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{c|c|c|c}
    \hline
    \textbf{Configuration} & \textbf{DeepSeek-MoE-16B} & \textbf{Mixtral-8x7B} & \textbf{DeepSeek-V2} \\
    \hline
    \textit{\# total params} & 16B & 47B & 236B \\
    \hline
    \textit{top-k} & 6 & 2 & 6\\
    \hline
    \textit{number of layers} & 28 & 32 & 60 \\
    \hline
    \textit{intermediate size} & 10944 & 4096 & 12288 \\
    \hline
    \textit{number of routed experts} & 64 & 8 & 160 \\
    \hline
    \textit{vocabulary size} & 102400 & 32000 & 102400 \\
    \hline
    \end{tabular}
    }
    \caption{Experimental Models Configurations.}
    \label{table:model-config}
    % \vspace{-15pt}
\end{table}

\subsection{Baselines and Metrics}\label{sec:expr:baselines}
We choose well-know LLM inference engines as baselines, listed as follows.

\paragraph{Huggingface TGI} The HuggingFace TGI Transformers (abbreviated as TGI) library is a powerful open-source tool designed for state-of-the-art machine learning. It provides a wide range of pre-trained models that can be used for various tasks across different modalities. HGT provide flexible APIs to serve large-scale transformer models using tensor parallelism. We choose HGT as a baseline to compare the native pytorch-implemented pure-TP MoE layers with \LTY.

\paragraph{vLLM} vLLM is a popular open-source LLM inference engine, adopting a bunch of optimization methods to boost the inference of transformer models, including but not limited to continuous batching, paged attention, flash attention, advanced quantization, etc. As for mixture-of-experts models, vLLM provides high-performance triton-kernels to enable purely TP implementation of fused gating-dispatching-computation process of the MoE layers. Another recently raising inference system, SGLang, delivers comparative (sometimes even better) performance compared with vLLM, in which the optimization mainly comes from RadixAttention while the MoE impelmentation is inherited from the vLLM MoE kernel. Thus, we select vLLM as the SOTA baseline to compare. The optimizations of the none-MoE parts are orthogonal to this paper. We test the performance of vLLM \LTY\ to prove \LTY's optimization effect against optimized MoE TP kernels.

\paragraph{DeepSpeed-MoE} DeepSpeed-MoE and its derivatives are strong baselines to deploy MoE models in large-scale clusters with hybrid parallelism including DP, TP and EP. \textbf{DeepSpeed-TED} is an optimized version of DeepSpeed-MoE, removing some of the redundant communications in MoE forward passing. \textbf{Tutel}~\cite{tutel} is a customized library to boost MoE training and inference that has been intergrated with DeepSpeed-MoE. We choose DeepSeek-TED (denoted as DeepSpeed-MoE or DS-MoE interchangeably), the advanced version of DeepSpeed-MoE (intergrating Tutel), as a strong comparable baseline to validate \LTY's optimization effect when facing sophisticated hybrid parallelism configurations in multi-server inference environment.

\paragraph{Metrics}
\LTY\ focuses on the speedup of the MoE layer when processing a large number of tokens, which is agnostic to prefilling and decoding. This is because the MoE layer is stateless and all the tokens of the same batch is flatten to a 2D tensor shaped like $[B \times S,d]$, where $B$, $S$, and $d$ are the batch size, sequence length and the hidden dimension. Thus, we sample different number of input prompts, defined by $B$, batch these prompts together, and measure the latency of the first token. For each $B$, we consecutively run $l$ loops with different input contents, recording the end-to-end time and per-batch time. We use the averaged per-batch time to calculate the \textit{latency} (ms) and the total number of tokens processed in $l$ loops divided by the end-to-end time as the \textit{throughput} (tokens per second) Furthermore, we set a latency service level objective (SLO) and compare the maximum throughput under this SLO. Similar to previous work~\cite{wu2024fastdistributedinferenceserving,wu2024loongserveefficientlyservinglongcontext}, we set SLO to 5$\times$ of the latency when number of tokens is 512. We adopt FP16 as the data format for model parameters and input tokens. Higher throughput and lower latency indicates better performance, as the orange arrow in the left-up corner of Figure~\ref{fig:ttft-e2e} and Figure~\ref{fig:ttft-e2e-multi} shows.

\subsection{Single-Node End-to-End Performance}\label{sec:expr:e2e}
Figure~\ref{fig:ttft-e2e} shows the optimization effect of \LTY\ on the 8-card L40S and 8-card H20 compared with baselines. For TGI,  vLLM and DS-MoE, we set the tensor parallelism degree as 8 to get the best performance (for DS-MoE, we select TP8 as the best configuration by comparing its performance under TP8/TP2EP4/TP4EP2/EP8). For \LTY, we adopt EP-8 configuration for DeepSeek-MoE-16B, DeepSeek-V2 and Mixtral-8x7B. As DS-MoE exhibits similar performance as TGI in single-node environment, we only report the performance of TGI here. The three figures of the first line reflect the performance of \LTY\ and baselines on the 8-card L40S server. For DeepSeek-MoE-16B, \LTY\ achieves upto 77.1\% and 51.2\% end-to-end latency reduction compared with TGI and vLLM. Under the pre-defined SLO, \LTY\ can reach 1.61x and 1.16x throughput compared with TGI and vLLM. For DeepSeek-V2, the boosting effect is similar, of which the latency reduction ratio and throughput increasing ratio are 76.8\%/68.8\% and 1.31x/1.15x. For Mixtral-8x7B, representing models with a small number of (relatively) larger experts, the speedup ratio is 76.7\%/65.8\% (latency reduction) and 1.28x/1.23x (throughput increasing), which mainly benefits from the fine-grained parallelism rather than the token-expert co-shuffling. Besides, TGI and vLLM yields similar performance for Mixtral-8x7B. This is because Mixtral-8x7B only contains 8 experts, of which only top-2 expert will be routed at runtime. Thus, a small number of experts would not benefit too much from the optimized grouped GEMM kernels in vLLM. The three figures in the second line depict the performance of the 8-card H20 server. The performance gain of Mixtral-8x7B is similar to that on the L40S server. The speedup effect of the DeepSeek family is slightly more significant. DeepSeek-MoE-16B can get up to 73.9\%/42.7\% end-to-end latency reduction while achieving a 4.14x/1.11x throughput increase compared with baselines. For DeepSeek-V2, the latency reduction ratio is 77.8\%/51.2\%, and the throughput boosting ratio is 3.10x/1.19x.


\begin{figure}[t]
    \centering
    \subfigure[Single-Node (8*L40S/8*H20).]{
    \label{fig:moe_breakdown:single}
    \includegraphics[width=.9\linewidth]{figures/moe-breakdown-single-v3.pdf}
    }
    \subfigure[Multi-Node (16 H100, 2 Nodes).]{
    \label{fig:moe_breakdown:multi}
    \includegraphics[width=.9\linewidth]{figures/moe-breakdown-multi-v3.pdf}
    }
    \caption{MoE layer performance breakdown.}
    \label{fig:moe_breakdown}
\end{figure}

\subsection{Multi-Node End-to-End Performance}\label{sec:expr:scaling}
We test the end-to-end performanece of DeepSeek-V2 and Mixtral-8x7B under multi-node environments. Figure~\ref{fig:ttft-e2e-multi} shows the optimization of \LTY\ on two-node H100 servers, compared with vLLM (TP16) and DeepSpeed-MoE (the optimized TED version and intergrated with Tutel) under different parallelism settings. Specifically, we select 4 typical parallelism configurations for each model, as depicted in the figure. For instance, DP2/TP8-EP2/TP8 indicates that the attention layer is sliced into 2 DP worlds, while parameters inside each DP world are partitioned into 8 TP slices. The MoE layer has 2 expert parallel groups, and experts inside each group are sharded into 8 TP slices. For DeepSeek-V2, we test the performance of \LTY, vLLM (TP16) and DS-MoE (using the same parallelism configuration as \LTY). Compared to vLLM-TP16/DS-MoE, \LTY\ gains 1.92x-6.90x/1.15x-7.72x throughput improvement and 41.4\%-82.2\%/13.7\%-93.0\% latency reduction as EP degree changes from 1 to 16. As the EP degree increases, the performance optimization effect becomes more significant. For Mixtral-8x7B, as its number of attention K/V heads is 8, TP16 can not be adopted to deploy the model. Thus we do not test the performance of vLLM-TP16 on it. When TP degree of the MoE layers equals 16, the performance of DS-MoE and \LTY\ are approximately the same. As EP size changes from 2 to 8, the throughput/latency optimization ratio varies from 1.56x-2.01x/54.9\%-70.0\%.

\subsection{MoE Layer Latency Breakdown}\label{sec:expr:breakdown}
\LTY\ is designed in a communication-efficient manner. Figure~\ref{fig:moe_breakdown} shows the communication latency breakdown of MoE layers of the DeepSeek-V2 model under single-node and multi-node environments.

In Figure~\ref{fig:moe_breakdown:single}, we draw the communication latency on single servers when the number of tokens is 16K and 32K. TGI and vLLM both adopt pure TP implementation, thus yiedling similar communication overhead. For DeepSeek-V2 under L40S and H20, \LTY\ gains $\sim$62.0\% and $\sim$40\% latency reduction. Figure~\ref{fig:moe_breakdown:multi} shows the inference latency breakdown of DeepSeek-V2 on 2 8*H100 servers. We measure the end-to-end latency undern two typical settings: attention with DP2/TP8 and MoE with EP2/TP8; attention with DP2/TP8 and MoE with EP16. The cross-server pure TP baseline incur heavy communication overhead due to dense \texttt{allreduce}. \LTY\ can achieve $\sim$20\% and $\sim$45\% communication latency reduction compared with vLLM in different parallelism settings. DS-MoE has bad performance under the DP2TP8-EP2TP8 setting, mainly attributed to cross-node \texttt{allgather} and \texttt{allreduce} caused by the EP-first layout. \LTY\ reduce the communication overhead by $\sim$70\% under this setting. Under DP2TP8-EP16 setting, DS-MoE delivers better performance, narrowing its gap against \LTY\ to $\sim$20\%.

\subsection{Ablation Study}\label{sec:expr:ablation}

We breakdown the performance improvement of \LTY\ via disabling the key features. Figure~\ref{fig:ablation} shows the ablation experiments on single-server environment compared with vLLM, describing the number of tokens can be processed under the SLO. The performance of the r-MoE outperforms baseline by 28.0\%/30.6\% and 60.0\%/64.1\% as for DeepSeek-MoE-16B/DeepSeek-V2 on 8*L40S server and 8*H20 server. On the L40S/H20 server, adding expert grouping (BX) and rebatching stage-1 (RB-s1, only considering the intra-layer conjugacy) brings $\sim$8.5\%/4.0\% and $\sim$9.0\%/4.5\% performance improvement. The improvement of applying rebatching stage-2 (RB-s2, considering both intra- and inter-layer conjugacy) is limited, which are $\sim$1.6\% and $\sim$1.2\% on L40S and H20.

To analyze the reason of communication speedup, Figure~\ref{fig:n_remote_act} shows the number of remote activation tokens of DeepSeek-MoE-16B and DeepSeek-V2 for different baselines. Each bar adds features to its left bar to show the optimization of the disassembly. With the help of the three optimization methods, the number of tokens sent to remote devices in \texttt{all2all} can be reduced by 41.94\%/43.38\%, which is the root cause of communication optimization.

\begin{figure}[t]
    \centering
    \subfigure[Performance Optimization Disassembling.]{
    \label{fig:ablation}
    \includegraphics[width=\linewidth]{figures/ablation-4D.pdf}
    }
    \subfigure[Optimization effect of number of remoted-activated tokens.]{
    \label{fig:n_remote_act}
    \includegraphics[width=\linewidth]{figures/n_remote_act.pdf}
    }
    \caption{Ablation study of \LTY. PB: piggybacking meta data with tokens. BX: expert grouping. RB: rebatching tokens. RB-s1: rebatching tokens with intra-layer conjugacy. RB-s2: rebtaching tokens with intra- and inter-layer conjugacy.}
    \label{fig:abl}
    % \vspace{-1cm}
\end{figure}

\subsection{Algorithm Evaluation}\label{sec:expr:algo}
\LTY\ adopts a cross-entropy-optimization-based (CEO-based) algorithm to approximately solve the token-expert co-clustering problem. We compare \LTY-CEO with some well-known baselines. Metis is a state-of-the-art graph partitioning algorithm that can generate partitions with minimal number of cross-partition edges, making it suitable for distributed message passing where the amount of network communication is proportional to the number of cross-partition edges. We adopt Metis in this scenario by abstracting the token-expert activation matrix as a bidirectional graph to find the minimum k-cut solution. Two-stage KMeans means performing KMeans-based clustering on the token-axis and expert-axis successively. Vanilla means that using the default expert/token layout without any shuffling. Figure~\ref{fig:algo_cmp} compares the four different solutions in the aspects of the local-activation rate ($\alpha$) and the load-balance rate ($\beta$), defined in \S~\ref{sec:parallel:perf}, in which \LTY-CEO can achieve the best localized actiavtion while guaranteeing load-balance.

==> method.tex <==
% \begin{figure*}[ht]
%     \centering
%     \includegraphics[width=0.9\linewidth]{figures/para_compared_with_baselines_v2.pdf}
%     \caption{Hybrid Attention-DP/TP + MoE-EP/TP in DeepSpeed.}
%     \label{fig:para_cmp}
% \end{figure*}

% \begin{table*}[t]
%     \centering
%     \resizebox{.9\linewidth}{!}{%
%     \begin{tabular}{c|c|c|c|c}
%     \hline
%     \textbf{Env.} & \textbf{Parallelism} & \textbf{Communication Pattern} & \textbf{Communication Volume} & \textbf{$\Delta$ Volume}\\ \hline
%     \multirow{2}{*}{\textbf{Single-Node}} & \textbf{TP} & \texttt{ar}-$G$/\texttt{ar}-$G$ & 
%     $S\left(\frac{4G-4}{G}\right)$ & \\ \cline{2-5}

%     & \textbf{r-MoE} & \texttt{rs}-$G$/\texttt{a2a}-$G$/\texttt{ag}-$G$ &
%     $S\left(\frac{2G-2}{G} + \frac{(1-\alpha)k}{G} \right)$ & $S\left(\frac{2G-2-(1-\alpha)k}{G}\right)$  \\ \hline
    
%     \multirow{2}{*}{\textbf{Multi-Node}} & \textbf{DS-MoE} & \texttt{ar}-$T_a$/\texttt{a2a}-$E$/\texttt{ag}-$T_e$/\texttt{ar}-$T_e$/\texttt{a2a}-$E$ &
%     $S\left(\frac{2T_a-2}{DT_a} + \frac{3T_e-3}{ET_e} + \frac{(2E-2)k}{E^2}\right)$ & \\ \cline{2-5}
    
%     % & \textbf{r-MoE (TP first)} & \texttt{rs}-$T_a$/\texttt{a2a}-$E$/\texttt{ag}-$T_e$/\texttt{rs}-$T_e$/\texttt{a2a}-$E$/\texttt{ag}-$T_a$ &
%     % $S\left(\frac{2T_a-2}{DT_a} + \frac{2T_e-2}{ET_e} + \frac{2(1-\frac{\alpha}{D})k}{E}\right)$ & 
%     % $S\left(\frac{T_e-1}{ET_e} + \frac{k}{E}\left(2\frac{\alpha}{D} - \frac{2}{E}\right)\right)$ \\ \cline{2-5}
    
%     & \textbf{r-MoE} & \texttt{rs}-$T_a$/\texttt{a2a}-$E$/\texttt{ag}-$T_e$/\texttt{rs}-$T_e$/\texttt{a2a}-$E$/\texttt{ag}-$T_a$ &
%     $S\left(\frac{2T_a-2}{DT_a} + \frac{2T_e-2}{ET_e} + \frac{2(1-\alpha)k}{E}\right)$ & 
%     $S\left(\frac{T_e-1}{ET_e} + \frac{k}{E}\left(2\alpha - \frac{2}{E} \right)\right)$ \\ \hline
%     \end{tabular}%
%     }
%     \caption{Communication volume comparison of different parallelism paradigms.}
%     \label{table:comm_cmp}
% \end{table*}
%\iffalse
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/workflow-en-v4.pdf}
    \caption{\LTY\ workflow}
    \label{fig:arch}
\end{figure}
%\fi
% \begin{figure*}[ht]
%     \centering
%     \includegraphics[width=\linewidth]{figures/icml-arch.pdf}
%     \caption{Speculative MoE Compared with Existing EP: illustration. $G$: number of GPUs. $B$: batch size. $S$: sequence length. $k$: topk. $\alpha$: local activation rate. A: Attention. AG: \texttt{allgather}. SRS: \texttt{shuffle-reduce-scatter}. A2A: \texttt{all2all}. E0/E1: expert 0/expert 1. TP-0/TP-1: tensor parallelism rank. The sizes of the components in the figure are disproportionate to the real run time of the operators.}
%     \label{fig:different-ep}
% \end{figure*}

\section{Methodology}

\subsection{Speculative MoE (s-MoE): Overview}

Figure~\ref{fig:arch} depicts the workflow of \LTY, in which the bold lines and dashed lines indicate online and offline operations, respectively. First, s-MoE collects token activation profiles, including token IDs and token-expert activation map (\normalsize{\textcircled{\small{1}}}\normalsize\enspace in Figure~\ref{fig:arch}). Using the co-clustering-based offline solver, s-MoE models token-expert affinity and computes experts shuffling tables $\mathcal{E}$ and lightweight lookup tables (including token-to-device table $\mathcal{T}$ and sequence-to-device $\mathcal{S}$ table). $\mathcal{E}$ is used to carry out speculative expert shuffling (s-EG) offline (\normalsize{\textcircled{\small{3}}}\normalsize\enspace in Figure~\ref{fig:arch}). $\mathcal{T}$ and $\mathcal{S}$ are leveraged by the \texttt{shuffled-reduce-scatter (SRS)} and \texttt{shuffled-allgather (SAG)} operator (i.e., speculative token shuffling (s-TS), \normalsize{\textcircled{\small{2}}}\normalsize\enspace in Figure~\ref{fig:arch}).

Figure~\ref{fig:illustration} depicts an illustrating example of how s-MoE works. In the baseline DS-MoE (the first row), tokens are synchronized by an \texttt{allreduce} operator and partially dropped before the gate module. After being decided which expert to activate, the tokens are sent to their corresponding devices for expert computation. Then the tokens are sent back, reduced locally, and gathered. After applying s-TS (the second row), the experts each token is routed to are predicted in advance before the gate module. Then the tokens are shuffled and scattered to their affiliative expert groups via the \texttt{SRS} operator ({\color{red}\normalsize{\textcircled{\small{1}}}\normalsize\enspace} in Figure~\ref{fig:illustration}), reducing the \texttt{all2all} communication volume via increasing local activation rate. Furthermore, when applying s-EG (the third row), experts are co-shuffled with tokens offline ({\color{red}\normalsize{\textcircled{\small{2}}}\normalsize\enspace} in Figure~\ref{fig:illustration}), enabling s-TS to achieve even higher local activation rate. In the example, the number of remote-activated tokens are trimmed from 5 to 3 to 1 after adopting s-TS and s-EG.
% The high performance of \LTY\ is guaranteed by the following two key designs.

% Firstly, \LTY\ employs \textit{speculative token shuffling} (s-TS). In modern LLM inference systems, tensor parallelism (TP) is commonly utilized to expedite attention computation. This necessitates an \texttt{allreduce (AR)} operation to synchronize all the partial computation results. When integrated with MoE-EP, \LTY\ substitutes the post-attention \texttt{allreduce} with a customized operator, \texttt{shuffle-reduce-scatter (SRS)}. \texttt{SRS} is a fused operator that combines local \texttt{shuffle} and \texttt{reduce-scatter} operations. The \texttt{shuffle} operation reorders the tokens based on the token - expert affinity hints. Given that \texttt{reduce-scatter (RS)} incurs only half of the communication overhead in comparison to \texttt{AR}, \texttt{SRS} systematically reduces the communication overhead in the attention layers, and strategically minimizes the \texttt{all2all} overhead in the MoE layers.

% Second, \LTY\ proposes \textit{speculative expert grouping}. \LTY\ computes the token-to-device (T2D) table, activation-sequence-to-device (S2D) table and expert-to-device (E2D) based on load-balance- and conjugacy-aware offline solver (\normalsize{\textcircled{\small{2}}}\normalsize\enspace in Figure~\ref{fig:arch}). The E2D table boxed conjugated experts in a single layer to eliminate dispersive activation while guaranteeing load-balance across expert groups (\normalsize{\textcircled{\small{3}}}\normalsize\enspace in Figure~\ref{fig:arch}). The T2D and S2D tables work together to aid in the online re-batching of tokens before each MoE layer, leveraging the intra-layer token-expert conjugacy and inter-layer expert conjugacy (\normalsize{\textcircled{\small{4}}}\normalsize\enspace in Figure~\ref{fig:arch}) to maximize localized activation. We detail the modeling method and offline/online algorithm in \S~\ref{sec:algo}.
% Second, \LTY\ proposes \textit{speculative expert grouping}. When $top\_k \geq 2$, the activated experts of a single token may distribute across different devices, limiting the optimization effect of speculative token shuffling. Taking the speculative token shuffling a step forward, \LTY\ furthermore models the token-expert affinity together via load-balance-aware co-clustering. \LTY\ computes the token-to-device (T2D) table, activation-sequence-to-device (S2D) table and expert-to-device (E2D) based on load-balance- and conjugacy-aware offline solver (\normalsize{\textcircled{\small{2}}}\normalsize\enspace in Figure~\ref{fig:arch}). The E2D table boxed conjugated experts in a single layer to eliminate dispersive activation while guaranteeing load-balance across expert groups (\normalsize{\textcircled{\small{3}}}\normalsize\enspace in Figure~\ref{fig:arch}). The T2D and S2D tables work together to aid in the online re-batching of tokens before each MoE layer, leveraging the intra-layer token-expert conjugacy and inter-layer expert conjugacy (\normalsize{\textcircled{\small{4}}}\normalsize\enspace in Figure~\ref{fig:arch}) to maximize localized activation.

% Secondly, \LTY\ puts forward \textit{speculative expert grouping} (s-EG). When $top\_k \geq 2$, the activated experts for a single token may be distributed across different devices, which restricts the optimization effect of speculative token shuffling. Building on the concept of speculative token shuffling, \LTY\ further models the token-expert affinity through load-balance-aware co-clustering.
% \LTY\ calculates the token-to-device (T2D) table, the activation-sequence-to-device (S2D) table, and the expert-to-device (E2D) table using a load-balance- and conjugacy-aware offline solver (as shown in \normalsize{\textcircled{\small{2}}}\normalsize\enspace in Figure~\ref{fig:arch}). The E2D table groups conjugated experts within a single layer. This not only eliminates scattered activation but also ensures load balance among expert groups (as depicted in \normalsize{\textcircled{\small{3}}}\normalsize\enspace in Figure~\ref{fig:arch}).
% The T2D and S2D tables collaborate to facilitate the online re-batching of tokens before each MoE layer. By leveraging the intra - layer token - expert conjugacy and inter-layer expert conjugacy (illustrated in \normalsize{\textcircled{\small{4}}}\normalsize\enspace in Figure~\ref{fig:arch}), they aim to maximize localized activation.

In the following subsections, we formulate the design of s-TS and s-EG in detail, and present an efficient algorithm to solve the optimal token/expert shuffling policy.

\subsection{Performance Analysis: Speculative Token Shuffling}\label{sec:parallel:formulation}
We derive the communication optimization principle of s-TS as follows. We use the symbol $\nu_{[...]}$ to represent the communication volume under hyper-parameters $[...]$.

\textbf{Preliminary \#1: communication volume of reduction collectives.} Suppose there are $G$ devices, the global batch size and the sequence are $B$ and $S$. The communication volume of \texttt{allreduce (AR)}, \texttt{allgather (AG)}, \texttt{reduce-scatter (RS)} is given by the following equations.

\begin{equation}
    \begin{aligned}
        &\nu_{G,B,S}(\texttt{AR}) = \frac{2(G-1)BS}{G} \\
        &\nu_{G,B,S}(\texttt{AG}) = \frac{(G-1)BS}{G} \\
        &\nu_{G,B,S}(\texttt{RS}) = \frac{(G-1)BS}{G}
    \end{aligned}
\end{equation}

\textbf{Preliminary \#2: communication volume of the p2p collective.} We define the percentage of tokens processed by local experts as the \textit{local activation rate} ($\alpha$, the percentage of tokens routed to local-hosted experts), and the number of experts each token is routed to is $k$. The communication volume of \texttt{all2all (A2A)} is given by the following equation.

\begin{equation}
    \nu_{G,B,S,k,\alpha}(\texttt{A2A}) = \frac{\alpha kBS}{G}
\end{equation}

Figure~\ref{fig:illustration} compares the s-TS design with DS-MoE using an illustration example. As we focus on the communication volume of attention TP and MoE EP. We implicitly suppose the DP degree of attention and the TP degree of MoE is 1. The communication pipeline of DS-MoE is \texttt{AR} $\rightarrow$ \texttt{A2A} $\rightarrow$ \texttt{A2A} $\rightarrow$ \texttt{AG}. We suppose the averaged local activation rate of the \texttt{A2A} in DS-MoE is $\frac{1}{G}$. Then the communication volume of DS-MoE-EP is given by: $\nu_{G,B,S}(\texttt{AR}) + 2\nu_{G,B,S,k,\frac{1}{G}}(\texttt{A2A}) + \nu_{G,B,S}(\texttt{AG}) = \frac{3BS(G-1)}{G} + \frac{2BSk(G-1)}{G^2} = BS(3-\frac{1}{G}-\frac{2}{G^2})$.

For s-MoE, the communication pipeline is \texttt{SRS} $\rightarrow$ \texttt{A2A} $\rightarrow$ \texttt{A2A}, and the communication volume is given by: $\nu_{G,B,S}(\texttt{RS}) + 2\nu_{G,B,S,k,\alpha}(\texttt{A2A})= \frac{BS(G-1)}{G} + \frac{2BSk(1-\alpha)}{G} = BS(1 + \frac{2k(1-\alpha) - 1}{G})$.

It can be derived that, the communication-saving volume of s-MoE compared with DS-MoE is $BS(2 - \frac{2k(1-\alpha)+\frac{2}{G}}{G})$. With local activation rate, $\alpha$, ranging from 0 to 1, the communication-saving volume ratio ranges from 32\%$\sim$75\%.

Thus, via speculative shuffling of tokens on the fly, a higher local activation rate can greatly trim the communication overhead. Together with the co-shuffling of experts, an even higher local activation rate could be achieved, which we will detail in the next subsection. 

\subsection{Co-shuffling Tokens and Experts}\label{sec:algo}

\begin{table}[t]
  \centering
  \resizebox{\linewidth}{!}{
  \begin{tabular}{c|c|c}
    \hline
    \textbf{Type} & \textbf{Symbol} & \textbf{Description} \\
    \hline
    \multirow{6}{*}{constants} & $t$ & \tabincell{c}{number of tokens collected in \\ offline profiling (deduplicated)} \\
    \cline{2-3}
    & $N$ & number of experts of a single MoE layer \\
    \cline{2-3}
    & $E$ & EP degree, also the number of clusters \\
    \cline{2-3}
    & $\bm{T}_{jk}$ & \tabincell{c}{times token $j$ activating expert $k$, \\ $\bm{T} \in \mathbb{N}^{t \times N}$} \\
    \cline{2-3}
    & $\bm{a}_j$ & \tabincell{c}{token $j$ frequency, \\ $\bm{a}_j = \sum_{k=1}^{N}\bm{T}_{jk},\ \bm{a} \in \mathbb{N}^{t}$} \\
    \cline{2-3}
    & $S$ & \tabincell{c}{number of tokens collected in \\ offline profiling (un-deduplicated), \\ $S=\sum_{j=1}^{t}\bm{a}_j$} \\
    \hline
    \multirow{2}{*}{decision variables} & $\bm{R}_{ij}$ & \tabincell{c}{whether token $j$ belongs to cluster $i$, \\ $\bm{R} \in \{0,1\}^{E \times t}$} \\
    \cline{2-3}
    & $\bm{C}_{ij}$ & \tabincell{c}{whether expert $j$ belongs to cluster $i$, \\ $\bm{C} \in \{0,1\}^{E \times N}$} \\
    \hline
  \end{tabular}
  }
  \caption{symbol and definition}
%   \vspace{-1cm}
  \label{table:notation}
\end{table}


\LTY\ applies conjugate parallelism (CJP) to realize token-expert affiliative activation, reducing \texttt{all2all} overhead. CJP models token-expert co-dispatching as a constrained co-clustering problem and generates the token-device scheduling table and expert-device scheduling table based on the token-expert activation table collected offline. Table ~\ref{table:notation} defines the symbols used by the algorithm and their definitions. Generally speaking, the algorithm tries to cluster tokens and experts at the same time so that tokens and experts in the same class have high local activation probability and ensure that the number of experts in each class is equal and the frequency of tokens in each class is as equal as possible to guarantee load-balance. The problem can be formally defined as a 0 - 1 integer programming (ILP) problem, as described in the following.

Hard constraints:
\begin{equation}\label{eq:constraints}
\begin{aligned}
&\sum_{i=1}^{E}\bm{R}_{ij} = 1,\ \text{for}\ j\ \text{from}\ 1\ \text{to}\ t \\
&\sum_{i=1}^{E}\bm{C}_{ij} = 1,\ \text{for}\ j\ \text{from}\ 1\ \text{to}\ N \\
&\sum_{j=1}^{N}\bm{C}_{ij} = \frac{N}{E},\ \text{for}\ i\ \text{from}\ 1\ \text{to}\ E
\end{aligned}
\end{equation}

Equation~\ref{eq:constraints} describes the hard constraints of this problem. From top to bottom, the constraints are: each token belongs to only one class, each expert belongs to only one class, and the number of experts in each class is equal.

There are two optimization objectives for this problem. The first objective is to ensure that the token frequencies of different clusters are as even as possible to ensure load balancing among EP ranks.
\begin{equation}\label{eq:load-balance}
\mathcal{L}_1 = \sum_{i=1}^{E}\left|\sum_{j=1}^{t}\left(\bm{R}_{ij}\bm{a}_j\right) - \frac{S}{E}\right|
\end{equation}

The second objective is to minimize the \texttt{all2all} communication overhead caused by remote activation (i.e., the summation of all the activations of tokens and experts belonging to different clusters).
\begin{equation}\label{eq:inter-device}
\mathcal{L}_2 = \sum_{i_1 \ne i_2}\left(\sum_{j=1}^{t}\sum_{k=1}^{N}\left(\bm{R}_{i_1j}\bm{C}_{i_2k}\bm{T}_{jk}\right)\right)
\end{equation}

The optimization objective can be defined as follows, controling the percentage of two sub-objectives using a factor $\theta$:
\begin{equation}\label{eq:obj}
\min: \mathcal{L} = \theta \mathcal{L}_1 + (1 - \theta) \mathcal{L}_2
\end{equation}

The ILP problem described in this section is difficult to solve directly using LP solvers. The reason is that a large number of intermediate variables are introduced in the linearization process, which leads to the dimension explosion of decision variables (please refer to the supplementary meterial for detailed analysis). \LTY\ provides a two-phase optimization algorithm based on the evolutionary algorithm. It can quickly obtain a feasible solution while ensuring load balancing. The next section describes the algorithm in detail.

% \begin{figure}[t]
% \centering
% \includegraphics[width=.9\linewidth]{figures/co_shf_example_v2.pdf}
% \caption{Example of token-expert conjugacy scheduling}
% \label{fig:co_shf_example}
% \end{figure}

\subsection{Methodology: Algorithm for the CJP Solver}\label{sec:algo:cem}
The Rubinstein Cross-Entropy Optimization (CEO) algorithm is a Monte Carlo method used primarily for optimization and importance sampling. Similar to the evolutionary algorithm, the CEO sprinkles points in space according to a certain rule, obtains the error of each point, and then determines the rule of the next round of sprinkle points according to the error information. The cross entropy method is named because the objective of the method (theoretically) is to minimize the cross entropy between the data distribution obtained by random scattered points and the actual data distribution (equivalent to minimizing the KL distance), trying to make the sampling distribution (sprinkling points) the same as the real distribution.

Algorithm ~\ref{algo:cem} describes the CEO-based token-expert co-scheduling algorithm in \LTY. The algorithm models each expert/token's choice of category as a D-dimensional polynomial distribution, and the probability of polynomial distribution is determined by $p\_matrix\_ep$ and $p\_matrix\_tk$ . Under the initial conditions, the probability of selecting each class by expert/token is set to equal. In each iteration, several class label samples are first sampled according to the probability matrix (lines 25-26). The sampling function \texttt{sample} samples label points from the D-dimensional polynomial distribution (line 11) and ensures that the number of experts in each category is equal (line 12-15). A relaxation factor $\beta$ is used to ensure that the token frequency of each category is as equal as possible (lines 16-19). After the sampling is complete, the algorithm calculates the local activation frequency of each sample (line 27) as the score, and selects samples with top-$\rho \times 100\%$ scores to update the probability matrix (line 27–line 28). After completing the $n\_steps$ iteration, the algorithm takes the cluster with the highest probability for each expert/token as its cluster label (lines 32-33). The clsuter label of expert/token actually represents the number of the device to which expert/token is scheduled. At the same time, the value of the probability matrix is used as the confidence that each token belongs to its cluster. In practice, the hyperparameters $\beta$ and $\rho$ are set as 1.1 and 0.2. By now, the token-device scheduling table $\mathcal{T}$, token-device scheduling confidence table $\mathcal{T}_p$, and expert-device scheduling table $\mathcal{E}$ are generated. After the scheduling table $\mathcal{E}$ is constructed, the experts at each layer need to be rearranged according to the scheduling table during online inference service deployment. In addition, the \LTY\ rearranges the gating module by column to implement transparent expert shuffle. The semantics of other layers are not affected. The rearranged experts are highly boxed, so that the token activation at each layer is de-cohesive, and the redundant network communication overhead caused by dispersive activation is reduced.

% Algorithm 1 in the supplementary material describes the CEO-based token-expert co-scheduling algorithm in \LTY. The algorithm models each expert/token's choice of category as a D-dimensional polynomial distribution, and the probability of polynomial distribution is determined by $p\_matrix\_ep$ and $p\_matrix\_tk$ . Under the initial conditions, the probability of selecting each class by expert/token is set to equal. In each iteration, several class label samples are first sampled according to the probability matrix. The sampling function \texttt{sample} samples label points from the D-dimensional polynomial distribution and ensures that the number of experts in each category is equal. A relaxation factor $\beta$ is used to ensure that the token frequency of each category is as equal as possible. After the sampling is complete, the algorithm calculates the local activation frequency of each sample as the score, and selects samples with top-$\rho \times 100\%$ scores to update the probability matrix. After completing the $n\_steps$ iteration, the algorithm takes the cluster with the highest probability for each expert/token as its cluster label. The clsuter label of expert/token actually represents the number of the device to which expert/token is scheduled. At the same time, the value of the probability matrix is used as the confidence that each token belongs to its cluster. In practice, the hyperparameters $\beta$ and $\rho$ are set as 1.1 and 0.2. By now, the token-device scheduling table $\mathcal{T}$, token-device scheduling confidence table $\mathcal{T}_p$, and expert-device scheduling table $\mathcal{E}$ are generated. After the scheduling table $\mathcal{E}$ is constructed, the experts at each layer need to be rearranged according to the scheduling table during online inference service deployment. In addition, the \LTY\ rearranges the gating module by column to implement transparent expert shuffle. The semantics of other layers are not affected. The rearranged experts are highly boxed, so that the token activation at each layer is de-cohesive, and the redundant network communication overhead caused by dispersive activation is reduced.

\begin{algorithm}[h!]
  \small
      \DontPrintSemicolon
      \caption{CEO-based co-clustering algorithm}
      \label{algo:cem}
      
      \SetKwFunction{FMIN}{min}
      \SetKwFunction{FOnes}{ones}
      \SetKwFunction{FSum}{sum}
      \SetKwFunction{FNorm}{norm}
      \SetKwFunction{FSample}{sample}
      \SetKwFunction{FLen}{len}
      \SetKwFunction{FArgmax}{argmax}
      \SetKwFunction{FIdmax}{argmax\_with\_values}

      \SetKwInput{Input}{input}\SetKwInput{Output}{output}
      
      \Input{$n\_steps$: number of iteration steps; $T$: token-expert activation matrix; $K$: number of samples of each sampling; $N$: number of experts per layer; $E$: number of co-clusters; $t$: number of tokens; $f$: token load-balance factor; $\rho$: percentage of tokens to choose during each iteration}
      \Output{$\mathcal{E}$: expert labels; $\mathcal{T}$: token labels; $\mathcal{T}_p$: confidence of tokens choosing specific experts}
      
      \SetKwProg{Fn}{Function}{:}{}
      
      $p\_matrix\_ep$ $\gets$ \FOnes{$N$, $E$} $/$ $E$
      
      $p\_matrix\_tk$ $\gets$ \FOnes{$t$, $E$} $/$ $E$

      \Fn{\FSample{$p\_matrix$, $n\_samples$, $type$, $\beta$}}{
          $samples$ $\gets$ empty list
          
          \Repeat{generated $n\_samples$ samples}{
              $mask$ $\gets$ \FOnes{$E$}
              
              $cnter$ $\gets$ hash map (default value is 0)
              
              $sample$ $\gets$ empty list
              
              \For{$i$ from $0$ to \FLen{$p\_matrix$}$ - 1$}{
                  $p$ $\gets$ \FNorm{$p\_matrix[i] * mask$}
                  
                  $cls$ $\gets$ sample a value from a multinomial distribution with $p$
                  
                  \If{$type$ is $expert$}{
                      $cnter[cls]$ $\gets$ $cnter[cls] + 1$
                      
                      \If{$cnter[cls]$ $==$ $E$}{
                          $mask[cls]$ $\gets$ 0
                      }
                  }
                  \If{$type$ is $token$}{
                      $cnter[cls]$ $\gets$ $cnter[cls] + $ \FSum{$T[i]$}
                      
                      \If{$cnter[cls]$ $>=$ \FSum{$T$} $/$ $E * \beta$}{
                          $mask[cls]$ $\gets$ 0
                      }
                  }
              }
              append $sample$ to $samples$
          }
          \KwRet{$samples$}
      }\;

      \Repeat{iterating for $n\_steps$ steps}{
          $ep\_samples$ $\gets$ \FSample{$p\_matrx\_ep$, $K$, $expert$}
          
          $tk\_samples$ $\gets$ \FSample{$p\_matrx\_tk$, $K$, $token$, $f$}
          
          $scores$ $\gets$ summation of $T$ of the same co-clusters
          
          $better\_samples$ $\gets$ samples with top-$\rho \times 100\%$ scores
          
          update $p\_matrix\_ep$ and $p\_matrix\_tk$
      }\;

      $\mathcal{E}$ $\gets$ \FArgmax{$p\_matrix\_ep$, axis=$1$}
      
      $\mathcal{T}$, $\mathcal{T}_p$ $\gets$ \FIdmax{$p\_matrix\_tk$, axis=$1$}\;
\end{algorithm}

\subsubsection{Extrapol $\mathcal{T}$ to the Full Vocabulary}
The token collected in offline profiling cannot cover all tokens in the model's vocabulary. Therefore, extrapolation of the scheduling table is required. \LTY\ calculates the cosine distance between token embeddings, associates token $\tau$ that is not covered by the profile with token $\tilde{\tau}$ appearing in the profile, and enables $\mathcal{T}[\tau]=\mathcal{T}[\tilde{\tau}]$ to extrapolate the token scheduling table.

\subsubsection{Modeling Inter-layer Activation Conjugacy}
Leveraging the conditional probability model described in \S~\ref{sec:bkg:token-expert}, we use a simple probability-based first-order Marcov chain to model the inter-layer activation conjugacy. To reduce the combination space, we model the activation device sequence rather than the activation expert sequence, because we only care about the device-level token rebatching. When looking back $l$ layers, we construct a table shaped like $[E^l, E]$, where the row of the table indicates the sequence of devices selected at the previous $l$ layers and the column indicates the probability of activating the $E$ devices in the current layer. Like the \S~\ref{sec:algo:cem} shows, we also calculate the activation sequence to device table $\mathcal{A}$ and the confidence table $\mathcal{A}_p$. In practice, we set the number of looking-back layers as 2.

\subsubsection{Re-batching on the Fly Based on Fast Lookup}

% We impelment a fast online re-batching mechanism based on fast looking-up tables. The algorithm queries the token-device scheduling table $\mathcal{T}$ and actiavtion-sequence-device table $\mathcal{S}$, together with their confidences first. Then, the table with higher confidence is adopted to obtain the device ID list to which the current batch token needs to be shuffle. The algorithm performs the argsort operation to obtain the shuffle indicators of the token. Then, the final shuffle indicators are obtained by grouping, aligning, and concatenation, and the token is shuffled. After rebatching is complete, \LTY\ calls the \texttt{reduce-scatter} operation. After MoE computing is complete, \LTY\ runs the \texttt{allgather} operation to collect tokens. Finally, the order of tokens are shuffled back based on the previously calculated shuffle indicators. The entire \texttt{rebatch} and \texttt{resume} processes do not involve load calculation and decision-making. They are directly completed by querying tables. The runtime overhead mainly involves large token matrix shuffling, which we optimize via high-performance kernels (refer to \S~\ref{sec:kernels}). The memory occupation of the scheduling tables is negligible. For example, for DeepSeek-V2, the memory space that the token-to-device table $\mathcal{T}$ occupies is $\frac{102400 \times 60 \times 2}{1024^2} \approx 11.72 MB$ (assuming the data format is \texttt{int16}). Please refer to the supplementary meterials for the detailed algorithm.

% \section{Detailed Online Re-rebatching Algorithm}

We implement a fast online re-batching mechanism based on fast looking-up tables (Algorithm~\ref{algo:fast_shf}). The algorithm queries the token-device scheduling table $\mathcal{T}$ and actiavtion-sequence-device table $\mathcal{S}$, together with their confidences first. Then, the table with higher confidence is adopted to obtain the device ID list to which the current batch token needs to be shuffle (line 2). The algorithm performs the argsort operation to obtain the shuffle indicators (line 3) of the token. Then, the final shuffle indicators are obtained by grouping, aligning, and concatenation, and the token is shuffled (line 4 to line 7). After rebatching is complete, \LTY\ calls the \texttt{reduce-scatter} operation. After MoE computing is complete, \LTY\ runs the \texttt{allgather} operation to collect tokens. Finally, the order of tokens are shuffled back based on the previously calculated shuffle indicators (lines 14-18). The entire \texttt{rebatch} and \texttt{resume} processes do not involve load calculation and decision-making. They are directly completed by querying tables. The runtime overhead mainly involves large token matrix shuffling, which we optimize via high-performance kernels. The memory occupation of the scheduling tables is negligible. For example, for DeepSeek-V2, the memory space that the token-to-device table $\mathcal{T}$ occupies is $\frac{102400 \times 60 \times 2}{1024^2} \approx 11.72 MB$ (assuming the data format is \texttt{int16}).

\begin{algorithm}[t]
  \small
  \DontPrintSemicolon
  \caption{Online re-batching based on fast lookup}
  \label{algo:fast_shf}
  
  \SetKwFunction{FSHF}{rebatch\_tokens}
  \SetKwFunction{FRES}{resume\_tokens}
  \SetKwFunction{FASORT}{argsort}
  \SetKwFunction{FALIGN}{align}
  \SetKwFunction{FGBK}{group\_by\_key}
  \SetKwFunction{FCAT}{concat}
  \SetKwFunction{FRS}{reduce\_scatter}
  \SetKwFunction{FAG}{allgather}
  \SetKwFunction{FCOND}{cond}
  
  \SetKwInput{Input}{input}\SetKwInput{Output}{output}
  
  \Input{$\mathcal{B} \in \mathbb{N}^{n}$: Input token IDs; $\mathcal{T}$: token-device Schedule Table}
  
  \SetKwProg{Fn}{Function}{:}{}
  
      \Fn{\FSHF{$\mathcal{B},\mathcal{T}$}}{
          % $dev\_ids\_T$ $\gets$ $\mathcal{T}\left[\mathcal{B}\right]$\;
          % $dev\_ids\_A$ $\gets$ $\mathcal{A}\left[\mathcal{B}\right]$\;
          $dev\_ids$ $\gets$ \FCOND{$\mathcal{T}_p\left[\mathcal{B}\right] > \mathcal{A}_p\left[\mathcal{B}\right]$, $\mathcal{T}\left[\mathcal{B}\right]$, $\mathcal{A}\left[\mathcal{B}\right]$}
          
          % \tcp*[l]{sort token IDs according to device IDs}
          $shf\_indices$ $\gets$ \FASORT{$dev\_ids$}
          
  
          % \tcp*[l]{group tokens according to device IDs}
          $g\_shf\_indices$ $\gets$ \FGBK{$shf\_indices$}
          
          % \tcp*[l]{align bins by round-robin picking-packing}
          $g\_shf\_indices$ $\gets$ \FALIGN{$g\_shf\_indices$}
          
          % \tcp*[l]{get the shuffle indices via concatting}
          $shf\_indices$ $\gets$ \FCAT{$g\_shf\_indices$}
          
          $\mathcal{B}$ $\gets$ $\mathcal{B}\left[shf\_indices\right]$
          
          \KwRet{$shf\_indices$}
      } \;
  
      \Fn{\FRES{$\mathcal{B},shf\_indices$}}{
          $r\_shf\_indices$ $\gets$ \FASORT{$shf\_indices$}
          
          $\mathcal{B}$ $\gets$ $\mathcal{B}\left[r\_shf\_indices\right]$
      } \;
  
      $shf\_indices$ $\gets$ \FSHF{$\mathcal{B},\mathcal{T}$}
      
      $\mathcal{B}_{local}$ $\gets$ \FRS{$\mathcal{B}$}
      
      executing MoE layer
      $\mathcal{B}$ $\gets$ \FAG{$\mathcal{B}_{local}$}
      
      \FRES{$\mathcal{B}$,$shf\_indices$}
  \end{algorithm}

==> method_lai.tex <==

\begin{figure}[t]
    \centering
    \includegraphics[width=.45\textwidth]{figures/workflow-en-v3.pdf}
    \caption{\LTY\ workflow}
    \label{fig:arch}
    \vspace{-0.6cm}
\end{figure}
%\fi
% \begin{figure*}[ht]
%     \centering
%     \includegraphics[width=\linewidth]{figures/icml-arch.pdf}
%     \caption{Speculative MoE Compared with Existing EP: illustration. $G$: number of GPUs. $B$: batch size. $S$: sequence length. $k$: topk. $\alpha$: local activation rate. A: Attention. AG: \texttt{allgather}. SRS: \texttt{shuffle-reduce-scatter}. A2A: \texttt{all2all}. E0/E1: expert 0/expert 1. TP-0/TP-1: tensor parallelism rank. The sizes of the components in the figure are disproportionate to the real run time of the operators.}
%     \label{fig:different-ep}
% \end{figure*}

\section{Methodology}

\subsection{Speculative MoE (s-MoE): Overview}

Figure~\ref{fig:arch} depicts the workflow of \LTY, in which the bold lines and dashed lines indicate online and offline operations, respectively. First, s-MoE collects token activation profiles, including token IDs and token-expert activation map (\normalsize{\textcircled{\small{1}}}\normalsize\enspace in Figure~\ref{fig:arch}). Using the co-clustering-based offline solver, s-MoE models token-expert affinity and computes experts shuffling tables $\mathcal{E}$ and lightweight lookup tables (including token-to-device table $\mathcal{T}$ and sequence-to-device $\mathcal{S}$ table). $\mathcal{E}$ is used to carry out speculative expert shuffling (s-EG) offline (\normalsize{\textcircled{\small{3}}}\normalsize\enspace in Figure~\ref{fig:arch}). $\mathcal{T}$ and $\mathcal{S}$ are leveraged by the \texttt{shuffled-reduce-scatter (SRS)} and \texttt{shuffled-allgather (SAG)} operator (i.e., speculative token shuffling (s-TS), \normalsize{\textcircled{\small{2}}}\normalsize\enspace in Figure~\ref{fig:arch}).

Figure~\ref{fig:illustration} depicts an illustrating example of how s-MoE works. In the baseline DS-MoE (the first row), tokens are synchronized by an \texttt{allreduce} operator and partially dropped before the gate module. After being decided which expert to activate, the tokens are sent to their corresponding devices for expert computation. Then the tokens are sent back, reduced locally, and gathered. After applying s-TS (the second row), the experts each token is routed to are predicted in advance before the gate module. Then the tokens are shuffled and scattered to their affiliative expert groups via the \texttt{SRS} operator ({\color{red}\normalsize{\textcircled{\small{1}}}\normalsize\enspace} in Figure~\ref{fig:illustration}), reducing the \texttt{all2all} communication volume via increasing local activation rate. Furthermore, when applying s-EG (the third row), experts are co-shuffled with tokens offline ({\color{red}\normalsize{\textcircled{\small{2}}}\normalsize\enspace} in Figure~\ref{fig:illustration}), enabling s-TS to achieve even higher local activation rate. In the example, the number of remote-activated tokens are trimmed from 5 to 3 to 1 after adopting s-TS and s-EG.

In the following subsections, we formulate the design of s-TS and s-EG in detail, and present an efficient algorithm to solve the optimal token/expert shuffling policy.


\subsection{Performance Analysis - s-TS and s-EG}\label{sec:parallel:formulation}
We derive the theoretical communication-saving volume from switching to the dynamic speculative schemes s-TS and s-EG as follows. 
% We derive the communication optimization principle of s-TS as follows. 
%\subsection{s-TS: from Deterministic to Speculative Scheme}\label{sec:parallel:formulation}
%We first derive the theoretical communication-saving volume from switching to the dynamic speculative scheme s-TS, and then detail how our proposed expert-routing forecasting model can improve the optimization effectiveness as follows. 
We use the symbol $\nu_{[...]}$ to represent the communication volume under hyper-parameters $[...]$.

\textbf{Preliminary1: communication volume of reduction collectives.} Suppose there are $G$ devices, the global batch size and the sequence are $B$ and $S$. The communication volume of \texttt{allreduce}, \texttt{allgather}, \texttt{reduce-scatter} is given by 
$\nu_{G,B,S}(\texttt{AR}) = \frac{2(G-1)BS}{G}$,
$\nu_{G,B,S}(\texttt{AG}) = \frac{(G-1)BS}{G}$,
$\nu_{G,B,S}(\texttt{RS}) = \frac{(G-1)BS}{G}$.
%\begin{equation}
%    \begin{aligned}
%        &\nu_{G,B,S}(\texttt{AR}) = \frac{2(G-1)BS}{G} \\
%        &\nu_{G,B,S}(\texttt{AG}) = \frac{(G-1)BS}{G} \\
%        &\nu_{G,B,S}(\texttt{RS}) = \frac{(G-1)BS}{G}
%    \end{aligned}
%\end{equation}

\textbf{Preliminary2: communication volume of the p2p collective.} We define the percentage of tokens processed by local experts as the \textit{local activation rate} ($\alpha$), and the number of experts each token is routed to is $k$. The communication volume of \texttt{all2all} is given by $\nu_{G,B,S,k,\alpha}(\texttt{A2A}) = \frac{\alpha kBS}{G}$.

Figure~\ref{fig:illustration} compares the s-MOE with DS-MoE. As we focus on the communication volume of attention TP and MoE EP. We implicitly suppose the DP degree of attention and the TP degree of MoE is 1. The communication pipeline of DS-MoE is \texttt{AR} $\rightarrow$ \texttt{A2A} $\rightarrow$ \texttt{A2A} $\rightarrow$ \texttt{AG}. We suppose the averaged local activation rate of the \texttt{A2A} in DS-MoE is $\frac{1}{G}$. Then the communication volume of DS-MoE-EP is given by: $\nu_{G,B,S}(\texttt{AR}) + 2\nu_{G,B,S,k,\frac{1}{G}}(\texttt{A2A}) + \nu_{G,B,S}(\texttt{AG}) = \frac{3BS(G-1)}{G} + \frac{2BSk(G-1)}{G^2} = BS(3-\frac{1}{G}-\frac{2}{G^2})$.

For s-MoE, the communication pipeline is \texttt{SRS} $\rightarrow$ \texttt{A2A} $\rightarrow$ \texttt{A2A}, and the communication volume is given by: $\nu_{G,B,S}(\texttt{RS}) + 2\nu_{G,B,S,k,\alpha}(\texttt{A2A})= \frac{BS(G-1)}{G} + \frac{2BSk(1-\alpha)}{G} = BS(1 + \frac{2k(1-\alpha) - 1}{G})$.

It can be derived that, the communication-saving volume of s-MoE compared with DS-MoE-EP and SGLang-EP are $BS(2 - \frac{2k(1-\alpha)+\frac{2}{G}}{G})$ and $BS(3-\frac{2k(1-\alpha) + 3}{G})$. With local activation rate, $\alpha$, ranging from 0 to 1, the communication-saving volume ratio ranges from 32\%$\sim$75\% and 16\%$\sim$69\%.

Therefore, a high local activation rate $\alpha$ can trim the communication overhead greatly, which can be achieved via properly co-clustering tokens and experts to the same device.
Our proposed s-MOE implements such idea by speculative shuffling of tokens on the fly by s-TS, together with the offline pre-grouping of experts from s-EG, to realize higher local activation rate, as detailed next. 

% Thus, via properly speculative shuffling of tokens on the fly, a higher local activation rate can trim the communication overhead greatly. 
% Together with the co-shuffling of experts, even higher local activation rate could be achieved.

% \textbf{Co-shuffling Tokens and Experts} 

%\subsection{Co-Clustering Tokens and Experts}\label{sec:algo}
\iffalse
We first propose a simple yet accurate probabilistic model to forecast expert routing paths. Leveraging this model, we formulate online token shuffling and offline expert pre-grouping simultaneously as an optimization problem to maximize the local activation rate. We then solve this problem using an efficient constrained cross-entropy method and generate lookup tables for fast online shuffling.
\fi

\subsection{Predicting Expert Routing Path}\label{sec:forecast-expert-routing}

% \subsection{Forecasting Expert Routing Paths via Tabulated Intra-Layer Token-Expert Conjugacy and Inter-Layer Expert Conjugacy}\label{sec:expert-routing}

% \subsubsection{Intra-layer token-expert affinity and Inter-layer expert-expert affinity} 

In general, the routing of token $x_j$ to $k$ experts in the $L^{th}$ MOE layer is governed by a gating network, expressed as
\[
G_{L}(h_{L,j}) = \texttt{top-k}(\texttt{softmax}(\mathbf{W}_{L,g} h_{L,j} + \mathbf{b}_{L,g})),
\]
where $h_{L,j}$ is the semantic representation of token $x_j$ processed by earlier layers along with its preceding tokens (context),
$\mathbf{W}_{L,g}$ and $\mathbf{b}_{L,g}$ are learnable parameters, 
and the \texttt{top-k} operation selects the $K$ most relevant experts. 
This formulation indicates that the selection of experts at layer $L$ is determined by both the token $x_j$ and its context, leading to an inherent \textbf{intra-layer token-expert affinity}.
Furthermore, the expert choices for $x_j$ in earlier layers are also determined by $x_j$ and its context, which subsequently influences the input to deeper layers.
Consequently, the expert choices at the $L^{th}$ layer exhibit an association with those in preceding layers, namely, \textbf{inter-layer expert-expert affinity}. 

%\textbf{Strong conjugacy between tokens/experts and experts regardless of the context.}
%We argue that, simple tabularized conditional probability model can work to predict
%the activation path of tokens implied by the above intra-layer/inter-layer affinity. 
%To show such feasibility, we further investigate both affinity phenomena empirically by conducting intermediate expert activation profiling experiments in the DeepSeek-MoE-16B and Mixtral-8x7B using the \textit{LongBench} dataset.
%On the one hand, we observe that semantically similar tokens are likely to activate
%a certain sub-group of experts as shown in Figure~\ref{fig:intra_layer_example}.
%The high kurtosis values for each token's activation map on the right part,
%further confirm that the to-route experts for each token concentrate on a narrowed set, regardless of the context.
%By using each tokens’ most routed top-k experts in partial (25\%) of the profile dataset to predict the activated experts in the remaining, we achieve a 96.3\% precision and a 78.8\% F1 score. 
%
%On the other hand, the left picture of Figure~\ref{fig:inter_layer_example} shows the activation correlation of the expert groups in the 4th and 5th layer of the Mixtral-8x7B model. For Mixtral-8x7B, each token is routed 2 out of 8 experts at each layer, resulting in ${8 \choose 2}=28$ expert groups. When tokens choose some concrete experts at the 4-th layer, they tend to choose a rather fixed set of experts at the next layer with high probability. 
%The right part of Figure~\ref{fig:inter_layer_example} shows that we can predict the activated top-k expert with confidence as high as 70\% by assigning the most frequent expert group followed by previous 5 layers.

%\textbf{Strong conjugacy between tokens/experts and experts regardless of the context.}
%We argue that a simple conditional probability model may suffice to predict the expert activation path of tokens implied by the above intra-layer/inter-layer affinity. We investigate both affinity phenomena empirically by conducting intermediate expert activation profiling experiments in the DeepSeek-MoE-16B and Mixtral-8x7B using the \textit{LongBench} dataset. Our results in Figure~\ref{fig:4d_affinity_example} of Appendix show that semantically similar tokens are likely to activate a certain sub-group of experts, regardless of the context. By using each tokens’ most routed top-k experts in partial (25\%) of the profile dataset to predict the activated experts in the remaining, we can achieve a 78.8\% F1 score. Moreover, when tokens choose some concrete experts at certain layers, they tend to choose a rather fixed set of experts at the next layer with high probability (70\% by assigning the most frequent expert group followed by previous 5 layers). 

\textbf{Simplified tabularized conditional probabilistic model for the gating network to forecast expert routing paths.}
We argue that a simple conditional probability model may suffice to predict the expert activation path of tokens implied by the above intra-layer/inter-layer affinity. We investigate both affinity phenomena empirically by conducting intermediate expert activation profiling experiments in the DeepSeek-MoE-16B and Mixtral-8x7B using the \textit{LongBench} dataset, as shown by Figure~\ref{fig:4d_affinity_example} of Appendix.
We find that semantically similar tokens are likely to activate a certain sub-group of experts, regardless of the context. Moreover, when tokens choose some concrete experts at certain layers, they tend to choose a rather fixed set of experts at the next layer with high probability. 

% Based on the above exploratory data analyses, we simplify \textbf{the modeling of intra-layer token-expert affinity},
Therefore,  we simplify \textbf{the modeling of intra-layer token-expert affinity},
using only the token $x_j$ to predict the probability of routing to $k$-th expert $E_{k}^{(L)}$ at the $L$-th MOE layer, 
$
\Pr(E^{(L)}_{k}|x_j)=\mathbf{T}^{(L)}_{j,k}/\sum_{k = 1}^{N^{(L)}}\mathbf{T}^{(L)}_{j,k},
\label{eq: pred_intra}
$
where $\mathbf{T}^{(L)}_{j,k}$ denotes the number of times the token $x_j$ is routed to the $k$-th expert $E^{(L)}_{k}$ within $L$-th MOE layer in the dataset collected during the offline profiling stage, for $j=1,\dots,t$ and $k=1,\dots,N^{(L)}$. 
For fast lookup of the matched expert for a given token, we tabularize the above token-expert relationship by \textbf{the token-2-expert confidence table} $\bm{\mathcal{A}}_p \in \mathbb{N}^{t \times N}$, where $\mathcal{A}_{p,jk}=\Pr(E_{k}|x_j)$
and we omit the layer index for representing the case in an arbitrary layer.
For an out-of-vocabulary (OOV) token $\tilde{x}$ not covered by the profile, we use the expert activation probabilities of the nearest known token $x'$ in the embedding space, measured by the cosine distance, as the prediction,
$
\Pr(E^{(L)}_{k}|\tilde{x}) \approx \Pr(E^{(L)}_{k} | x'), \text{where } x' = \arg\min_{x} \text{DIST}_{cos}(\tilde{x},x),
$
which ensures robust predictions even for OOV tokens.

To simplify \textbf{modeling inter-layer expert-expert affinity},
because we only care about the device-level token shuffling,
we model the coarser activation device sequence rather than the activation expert sequence with a $n$-gram model $\Pr(D^{(L)}_{k}|D^{(L-1)}, \ldots, D_{(L-n)})$ where $D_{(l)}\in\{1,\ldots,Q\}$ denote the device index where the chosen expert locates at the $l$-th layer for an arbitrary token.
We also tabularize the above expert-expert relationship via 
a sequence-2-device confidence table $\mathcal{B}_p \in \mathbb{N}^{Q^n \times Q}$ and the corresponding sequence-2-device table  $\mathcal{B}=\text{argmax}(\mathcal{B}_p, \text{axis}=1) \in \mathbb{N}^{Q^n \times 1}$. We use 2-gram in practice.
Together, the expert routing paths can be predicted accurately by either the intra-layer token-expert model or inter-layer expert-expert model. 

\subsection{Balanced Token-Expert Co-clustering}\label{sec:ilp}

We illustrate how such expert-routing forecasting models can guide the co-dispatching of tokens and experts. 
Instead to existed solving method such as Metis and two-stage Kmeans, 
\LTY\ models the token-expert co-clustering problem as a 0 - 1 integer programming (ILP) problem.

From the offline profling, we obtain the number of deduplicated (un-deduplicated) tokens $t$ ($S$), the number of expert per layer $N$, the the number of clusters $E$ (also EP degree), 
the token $j$ frequency $\bm{a}_j$, and the predicted probability $\bm{\mathcal{A}}_{p,jk}$ that token $j$ activates expert $k$.
The decision integer variables are set as the placement $\bm{R}_{ij}\in\{0,1\}$ of token $j$ to cluster $i$ and the placement $\bm{C}_{ij}\in\{0,1\}$ of expert $j$ to cluster $i$.
We aim to minimize an objective function
$\mathcal{L} = \theta \sum_{i=1}^{E}\left|\sum_{j=1}^{t}\left(\bm{R}_{ij}\bm{a}_j\right) - \frac{S}{E}\right| + (1 - \theta) \sum_{i_1 \ne i_2}\left(\sum_{j=1}^{t}\sum_{k=1}^{N}\left(\bm{R}_{i_1j}\bm{C}_{i_2k}\bm{\mathcal{A}}_{p,jk}\right)\right)$, where the left part is to ensure that the token frequencies of different clusters as even as possible to promote load balancing among EP ranks, and the right part is to minimize the 
\texttt{all2all} communication overhead caused by remote activation (i.e., the summation of all the activations of tokens and experts belonging to different clusters), a factor $\theta\in (0,1)$  controling the percentage of two sub-objectives.
We further require that each token belongs to only one class, each expert belongs to only one class, and the number of experts in each class is equal by adding hard constraints 
$\sum_{i=1}^{E}\bm{R}_{ij} = 1,\ \text{for}\ j= 1 \dots t$,
$\sum_{i=1}^{E}\bm{C}_{ij} = 1,\ \text{for}\ j= 1 \dots N$,
and $\sum_{j=1}^{N}\bm{C}_{ij} = \frac{N}{E},\ i= 1 \dots t$.

% Equation~\ref{eq:obj} computes the objective function where the left part is to ensure that the token frequencies of different clusters as even as possible to promote load balancing among EP ranks, and the right part is to minimize the 
% \texttt{all2all} communication overhead caused by remote activation (i.e., the summation of all the activations of tokens and experts belonging to different clusters), a factor $\theta\in (0,1)$  controling the percentage of two sub-objectives.
% Equation~\ref{eq:constraints} describes the hard constraints of this problem. From top to bottom, the constraints are: each token belongs to only one class, each expert belongs to only one class, and the number of experts in each class is equal.

% \begin{align}
% \text{Minimize} \quad & \mathcal{L} = \theta \sum_{i=1}^{E}\left|\sum_{j=1}^{t}\left(\bm{R}_{ij}\bm{a}_j\right) - \frac{S}{E}\right| + \notag \\
% \quad & (1 - \theta) \sum_{i_1 \ne i_2}\left(\sum_{j=1}^{t}\sum_{k=1}^{N}\left(\bm{R}_{i_1j}\bm{C}_{i_2k}\bm{T}_{jk}\right)\right) \label{eq:obj}\\
% \text{Variable} \quad & \bm{R}_{i, j} \in \{0, 1\}, \bm{C}_{i,j} \in \{0, 1\}\label{eq:var} \\
% \text{Subject to} \quad &\sum_{i=1}^{E}\bm{R}_{ij} = 1,\ \text{for}\ j\ \text{from}\ 1\ \text{to}\ t, \notag \\ 
% &\sum_{i=1}^{E}\bm{C}_{ij} = 1,\ \text{for}\ j\ \text{from}\ 1\ \text{to}\ N \label{eq:constraints} \\ 
% &\sum_{j=1}^{N}\bm{C}_{ij} = \frac{N}{E},\ \text{for}\ i\ \text{from}\ 1\ \text{to}\ E \notag
% \end{align}

The above ILP problem is difficult to solve directly using LP solvers, given a large number of intermediate variables introduced in the linearization process. \LTY\ provides a two-phase cross-entropy optimization algorithm. 
It can quickly obtain a feasible solution while ensuring load balancing. The detailed co-clustering algorithm can be referred to in \S~\ref{sec:algo:cem} in the Appendix. The solution can then be applied to online speculative token shuffling and offline speculative expert grouping, which can be referred to in \S~\ref{sec:algo:cem} as well.

%\begin{figure}[t]
%\centering
%\includegraphics[width=.9\linewidth]{figures/co_shf_example_v2.pdf}
%\caption{Example of token-expert conjugacy scheduling}
%\label{fig:co_shf_example}
%\end{figure}



==> method_lai2.tex <==

\begin{figure}[htbp]
    \centering
    \includegraphics[width=.4\textwidth]{figures/workflow-en-v4.pdf}
    \caption{\LTY\ workflow}
    \label{fig:arch}
    \vspace{-0.6cm}
\end{figure}
%\fi
% \begin{figure*}[ht]
%     \centering
%     \includegraphics[width=\linewidth]{figures/icml-arch.pdf}
%     \caption{Speculative MoE Compared with Existing EP: illustration. $G$: number of GPUs. $B$: batch size. $S$: sequence length. $k$: topk. $\alpha$: local activation rate. A: Attention. AG: \texttt{allgather}. SRS: \texttt{shuffle-reduce-scatter}. A2A: \texttt{all2all}. E0/E1: expert 0/expert 1. TP-0/TP-1: tensor parallelism rank. The sizes of the components in the figure are disproportionate to the real run time of the operators.}
%     \label{fig:different-ep}
% \end{figure*}

\section{Methodology}

\subsection{Speculative MoE (s-MoE): Overview}

Figure~\ref{fig:arch} shows \LTY's workflow, in which the bold lines and dashed lines indicate online and offline operations. First, s-MoE collects token activation profiles, including token IDs and token-expert activation frequencies (\normalsize{\textcircled{\small{1}}}\normalsize\enspace in Figure~\ref{fig:arch}). s-MoE probabilistically models the token-expert routing likelihood and solves a balanced token-expert co-clustering problem to make the co-scheduling hints, which includes lightweight lookup tables (token-to-expert-cluster table $\mathcal{T}$, and expert-cluster-sequence-to-expert-cluster table $\mathcal{S}$) and experts grouping tables $\mathcal{E}$. Tables $\mathcal{T}$ and $\mathcal{S}$ are used by the \texttt{shuffled-reduce-scatter (SRS)} and \texttt{shuffled-allgather (SAG)} kernel (i.e., speculative token shuffling, s-TS, \normalsize{\textcircled{\small{2}}}\normalsize\enspace in Figure~\ref{fig:arch}). $\mathcal{E}$ is used for speculative expert shuffling, s-EG (\normalsize{\textcircled{\small{3}}}\normalsize\enspace in Figure~\ref{fig:arch}).

Figure~\ref{fig:illustration} depicts an illustrating example of how s-MoE works. In the baseline DS-MoE (the first row), tokens are synchronized by an \texttt{allreduce} operator and partially dropped before the gate module. After being decided which expert to activate, the tokens are sent to their corresponding devices for expert computation. Then the tokens are sent back, reduced locally, and gathered. After applying s-TS (the second row), the experts each token is routed to are predicted in advance before the gate module. Then the tokens are shuffled and scattered to their affiliative expert groups via the \texttt{SRS} operator ({\color{red}\normalsize{\textcircled{\small{1}}}\normalsize\enspace} in Figure~\ref{fig:illustration}), reducing the \texttt{all2all} communication volume via increasing local activation rate. Furthermore, when applying s-EG (the third row), experts are co-shuffled with tokens offline ({\color{red}\normalsize{\textcircled{\small{2}}}\normalsize\enspace} in Figure~\ref{fig:illustration}), enabling s-TS to achieve even higher local activation rate. In the example, the number of remote-activated tokens are trimmed from 5 to 3 to 1 after adopting s-TS and s-EG. We detail the performance analysis and algorithms of s-TS and s-EG in the following subsections.

\subsection{Performance Analysis - s-TS and s-EG}\label{sec:parallel:formulation}
We derive the theoretical communication-saving volume from switching to the dynamic speculative schemes s-TS and s-EG as follows. 
% We derive the communication optimization principle of s-TS as follows. 
%\subsection{s-TS: from Deterministic to Speculative Scheme}\label{sec:parallel:formulation}
%We first derive the theoretical communication-saving volume from switching to the dynamic speculative scheme s-TS, and then detail how our proposed expert-routing forecasting model can improve the optimization effectiveness as follows. 
We use the symbol $\nu_{[...]}$ to represent the communication volume under hyper-parameters $[...]$.

\textbf{Preliminary1: communication volume of reduction collectives.} Suppose there are $G$ devices, the global batch size and the sequence are $B$ and $S$. The communication volume of \texttt{allreduce}, \texttt{allgather}, \texttt{reduce-scatter} is given by 
$\nu_{G,B,S}(\texttt{AR}) = \frac{2(G-1)BS}{G}$,
$\nu_{G,B,S}(\texttt{AG}) = \frac{(G-1)BS}{G}$,
$\nu_{G,B,S}(\texttt{RS}) = \frac{(G-1)BS}{G}$.

\textbf{Preliminary2: communication volume of the p2p collective.} We define the percentage of tokens processed by local experts as the \textit{local activation rate} ($\alpha$), and the number of experts each token is routed to is $k$. The communication volume of \texttt{all2all} is given by $\nu_{G,B,S,k,\alpha}(\texttt{A2A}) = \frac{\alpha kBS}{G}$.

Figure~\ref{fig:illustration} compares the s-MOE with DS-MoE. As we focus on the communication volume of attention TP and MoE EP. We implicitly suppose the DP degree of attention and the TP degree of MoE is 1. The communication pipeline of DS-MoE is \texttt{AR} $\rightarrow$ \texttt{A2A} $\rightarrow$ \texttt{A2A} $\rightarrow$ \texttt{AG}. We suppose the averaged local activation rate of the \texttt{A2A} in DS-MoE is $\frac{1}{G}$. Then the communication volume of DS-MoE-EP is given by: $\nu_{G,B,S}(\texttt{AR}) + 2\nu_{G,B,S,k,\frac{1}{G}}(\texttt{A2A}) + \nu_{G,B,S}(\texttt{AG}) = \frac{3BS(G-1)}{G} + \frac{2BSk(G-1)}{G^2} = BS(3-\frac{1}{G}-\frac{2}{G^2})$.

For s-MoE, the communication pipeline is \texttt{SRS} $\rightarrow$ \texttt{A2A} $\rightarrow$ \texttt{A2A}, and the communication volume is given by: $\nu_{G,B,S}(\texttt{RS}) + 2\nu_{G,B,S,k,\alpha}(\texttt{A2A})= \frac{BS(G-1)}{G} + \frac{2BSk(1-\alpha)}{G} = BS(1 + \frac{2k(1-\alpha) - 1}{G})$.

It can be derived that, the communication-saving volume of s-MoE compared with DS-MoE-EP and SGLang-EP are $BS(2 - \frac{2k(1-\alpha)+\frac{2}{G}}{G})$ and $BS(3-\frac{2k(1-\alpha) + 3}{G})$. With local activation rate, $\alpha$, ranging from 0 to 1, the communication-saving volume ratio ranges from 32\%$\sim$75\% and 16\%$\sim$69\%.

Therefore, a high local activation rate $\alpha$ can trim the communication overhead greatly, which can be achieved via properly co-clustering tokens and experts to the same device.
Our proposed s-MOE implements such an idea by speculatively shuffling of tokens on the fly by s-TS, together with the offline pre-grouping of experts from s-EG, to realize a higher local activation rate, as detailed next. 

% Thus, via properly speculative shuffling of tokens on the fly, a higher local activation rate can trim the communication overhead greatly. 
% Together with the co-shuffling of experts, even higher local activation rate could be achieved.

% \textbf{Co-shuffling Tokens and Experts} 

%\subsection{Co-Clustering Tokens and Experts}\label{sec:algo}
\iffalse
We first propose a simple yet accurate probabilistic model to forecast expert routing paths. Leveraging this model, we formulate online token shuffling and offline expert pre-grouping simultaneously as an optimization problem to maximize the local activation rate. We then solve this problem using an efficient constrained cross-entropy method and generate lookup tables for fast online shuffling.
\fi

\subsection{Predicting Expert Routing Path}\label{sec:forecast-expert-routing}

% \subsection{Forecasting Expert Routing Paths via Tabulated Intra-Layer Token-Expert Conjugacy and Inter-Layer Expert Conjugacy}\label{sec:expert-routing}

% \subsubsection{Intra-layer token-expert affinity and Inter-layer expert-expert affinity} 

In general, the routing of token $x_j$ to $k$ experts in the $L^{th}$ MOE layer is governed by a gating network, expressed as
\[
G_{L}(h_{L,j}) = \texttt{top-k}(\texttt{softmax}(\mathbf{W}_{L,g} h_{L,j} + \mathbf{b}_{L,g})),
\]
where $h_{L,j}$ is the semantic representation of token $x_j$ processed by earlier layers along with its preceding tokens (context),
$\mathbf{W}_{L,g}$ and $\mathbf{b}_{L,g}$ are learnable parameters, 
and the \texttt{top-k} operation selects the $K$ most relevant experts. 
This formulation indicates that the selection of experts at layer $L$ is determined by both the token $x_j$ and its context, leading to an inherent \textbf{intra-layer token-expert affinity}.
Furthermore, the expert choices for $x_j$ in earlier layers are also determined by $x_j$ and its context, which subsequently influences the input to deeper layers.
Consequently, the expert choices at the $L^{th}$ layer exhibit an association with those in preceding layers, namely, \textbf{inter-layer expert-expert affinity}. 

%\textbf{Strong conjugacy between tokens/experts and experts regardless of the context.}
%We argue that, simple tabularized conditional probability model can work to predict
%the activation path of tokens implied by the above intra-layer/inter-layer affinity. 
%To show such feasibility, we further investigate both affinity phenomena empirically by conducting intermediate expert activation profiling experiments in the DeepSeek-MoE-16B and Mixtral-8x7B using the \textit{LongBench} dataset.
%On the one hand, we observe that semantically similar tokens are likely to activate
%a certain sub-group of experts as shown in Figure~\ref{fig:intra_layer_example}.
%The high kurtosis values for each token's activation map on the right part,
%further confirm that the to-route experts for each token concentrate on a narrowed set, regardless of the context.
%By using each tokens’ most routed top-k experts in partial (25\%) of the profile dataset to predict the activated experts in the remaining, we achieve a 96.3\% precision and a 78.8\% F1 score. 
%
%On the other hand, the left picture of Figure~\ref{fig:inter_layer_example} shows the activation correlation of the expert groups in the 4th and 5th layer of the Mixtral-8x7B model. For Mixtral-8x7B, each token is routed 2 out of 8 experts at each layer, resulting in ${8 \choose 2}=28$ expert groups. When tokens choose some concrete experts at the 4-th layer, they tend to choose a rather fixed set of experts at the next layer with high probability. 
%The right part of Figure~\ref{fig:inter_layer_example} shows that we can predict the activated top-k expert with confidence as high as 70\% by assigning the most frequent expert group followed by previous 5 layers.

%\textbf{Strong conjugacy between tokens/experts and experts regardless of the context.}
%We argue that a simple conditional probability model may suffice to predict the expert activation path of tokens implied by the above intra-layer/inter-layer affinity. We investigate both affinity phenomena empirically by conducting intermediate expert activation profiling experiments in the DeepSeek-MoE-16B and Mixtral-8x7B using the \textit{LongBench} dataset. Our results in Figure~\ref{fig:4d_affinity_example} of Appendix show that semantically similar tokens are likely to activate a certain sub-group of experts, regardless of the context. By using each tokens’ most routed top-k experts in partial (25\%) of the profile dataset to predict the activated experts in the remaining, we can achieve a 78.8\% F1 score. Moreover, when tokens choose some concrete experts at certain layers, they tend to choose a rather fixed set of experts at the next layer with high probability (70\% by assigning the most frequent expert group followed by previous 5 layers). 

\textbf{Simplified tabularized conditional probabilistic model for the gating network to forecast expert routing paths.}
We argue that a simple conditional probability model may suffice to predict the expert activation path of tokens implied by the above intra-layer/inter-layer affinity. We investigate both affinity phenomena empirically by conducting intermediate expert activation profiling experiments in the DeepSeek-MoE-16B and Mixtral-8x7B using the \textit{LongBench} dataset, as shown by Figure~\ref{fig:4d_affinity_example} of Appendix.
We find that semantically similar tokens are likely to activate a certain sub-group of experts, regardless of the context. Moreover, when tokens choose some concrete experts at certain layers, they tend to choose a rather fixed set of experts at the next layer with high probability.

Therefore,  we simplify \textbf{the modeling of intra-layer token-expert affinity},
using only the token $x_j$ to predict the probability of routing to $k$-th expert $E_{k}^{(L)}$ at the $L$-th MOE layer, 
$
\Pr(E^{(L)}_{k}|x_j)=\mathbf{T}^{(L)}_{j,k}/\sum_{k = 1}^{N^{(L)}}\mathbf{T}^{(L)}_{j,k},
\label{eq: pred_intra}
$
where $\mathbf{T}^{(L)}_{j,k}$ denotes the number of times the token $x_j$ is routed to the $k$-th expert $E^{(L)}_{k}$ within $L$-th MOE layer in the dataset collected during the offline profiling stage, for $j=1,\dots,t$ and $k=1,\dots,N^{(L)}$. 
For fast lookup of the matched expert for a given token, we tabularize the above token-expert relationship by \textbf{the token-2-expert confidence table} $\bm{\mathcal{C}}_p \in \mathbb{N}^{t \times N}$, where $\mathcal{C}_{p,jk}=\Pr(E_{k}|x_j)$
and we omit the layer index for representing the case in an arbitrary layer.
For an out-of-vocabulary (OOV) token $\tilde{x}$ not covered by the profile, we use the expert activation probabilities of the nearest known token $x'$ in the embedding space, measured by the cosine distance, as the prediction,
% $
% \Pr(E^{(L)}_{k}|\tilde{x}) \approx \Pr(E^{(L)}_{k} | x'), \text{where } x' = \arg\min_{x} \text{DIST}_{cos}(\tilde{x},x),
% $
which ensures robust predictions even for OOV tokens.

To simplify \textbf{modeling inter-layer expert-expert affinity},
because we only care about the device-level token shuffling,
we model the coarser activation expert cluster sequence rather than the activation expert sequence with a $n$-gram model $\Pr(D^{(L)}_{k}|D^{(L-1)}, \ldots, D_{(L-n)})$ where $D_{(l)}\in\{1,\ldots,Q\}$ denote the device index where the chosen expert locates at the $l$-th layer for an arbitrary token.
We also tabularize the above expert-expert relationship via 
a expert-cluster-sequence-2-expert-cluster confidence table $\mathcal{A}_p \in \mathbb{N}^{Q^n \times Q}$ and the corresponding expert-cluster-sequence-2-expert-cluster table  $\mathcal{A}=\text{argmax}(\mathcal{A}_p, \text{axis}=1) \in \mathbb{N}^{Q^n \times 1}$. We use 2-gram in practice.
Together, the expert routing paths can be predicted accurately by either the intra-layer token-expert model or inter-layer expert-expert model. 

\subsection{Balanced Token-Expert Co-clustering}\label{sec:ilp}

We illustrate how such expert-routing forecasting models can guide the co-dispatching of tokens and experts. 
Different from existing solvers such as Metis and two-stage Kmeans, 
\LTY\ models the token-expert co-clustering problem as a 0 - 1 integer programming (ILP) problem.

From the offline profiling, we obtain the number of deduplicated (un-deduplicated) tokens $t$ ($S$), the number of experts per layer $N$, the number of clusters $E$ (also EP degree), 
the token $j$ frequency $\bm{a}_j$, and the predicted probability $\bm{\mathcal{C}}_{p,jk}$ that token $j$ activates expert $k$.
The decision integer variables are set as the placement $\bm{R}_{ij}\in\{0,1\}$ of token $j$ to cluster $i$ and the placement $\bm{C}_{ij}\in\{0,1\}$ of expert $j$ to cluster $i$.
We aim to minimize an objective function
$\mathcal{L} = \theta \sum_{i=1}^{E}\left|\sum_{j=1}^{t}\left(\bm{R}_{ij}\bm{a}_j\right) - \frac{S}{E}\right| + (1 - \theta) \sum_{i_1 \ne i_2}\left(\sum_{j=1}^{t}\sum_{k=1}^{N}\left(\bm{R}_{i_1j}\bm{C}_{i_2k}\bm{\mathcal{C}}_{p,jk}\bm{a}_j\right)\right)$, where the left part is to ensure that the token frequencies of different clusters as even as possible to promote load balancing among EP ranks, and the right part is to minimize the 
\texttt{all2all} communication overhead caused by remote activation (i.e., the summation of all the activations of tokens and experts belonging to different clusters), a factor $\theta\in (0,1)$  controlling the percentage of two sub-objectives.
We further require that each token belongs to only one class, each expert belongs to only one class, and the number of experts in each class is equal by adding hard constraints 
$\sum_{i=1}^{E}\bm{R}_{ij} = 1,\ \text{for}\ j= 1 \dots t$,
$\sum_{i=1}^{E}\bm{C}_{ij} = 1,\ \text{for}\ j= 1 \dots N$,
and $\sum_{j=1}^{N}\bm{C}_{ij} = \frac{N}{E},\ i= 1 \dots t$.

% Equation~\ref{eq:obj} computes the objective function where the left part is to ensure that the token frequencies of different clusters as even as possible to promote load balancing among EP ranks, and the right part is to minimize the 
% \texttt{all2all} communication overhead caused by remote activation (i.e., the summation of all the activations of tokens and experts belonging to different clusters), a factor $\theta\in (0,1)$  controling the percentage of two sub-objectives.
% Equation~\ref{eq:constraints} describes the hard constraints of this problem. From top to bottom, the constraints are: each token belongs to only one class, each expert belongs to only one class, and the number of experts in each class is equal.

% \begin{align}
% \text{Minimize} \quad & \mathcal{L} = \theta \sum_{i=1}^{E}\left|\sum_{j=1}^{t}\left(\bm{R}_{ij}\bm{a}_j\right) - \frac{S}{E}\right| + \notag \\
% \quad & (1 - \theta) \sum_{i_1 \ne i_2}\left(\sum_{j=1}^{t}\sum_{k=1}^{N}\left(\bm{R}_{i_1j}\bm{C}_{i_2k}\bm{T}_{jk}\right)\right) \label{eq:obj}\\
% \text{Variable} \quad & \bm{R}_{i, j} \in \{0, 1\}, \bm{C}_{i,j} \in \{0, 1\}\label{eq:var} \\
% \text{Subject to} \quad &\sum_{i=1}^{E}\bm{R}_{ij} = 1,\ \text{for}\ j\ \text{from}\ 1\ \text{to}\ t, \notag \\ 
% &\sum_{i=1}^{E}\bm{C}_{ij} = 1,\ \text{for}\ j\ \text{from}\ 1\ \text{to}\ N \label{eq:constraints} \\ 
% &\sum_{j=1}^{N}\bm{C}_{ij} = \frac{N}{E},\ \text{for}\ i\ \text{from}\ 1\ \text{to}\ E \notag
% \end{align}

The above ILP problem is difficult to solve directly using LP solvers, given a large number of intermediate variables introduced in the linearization process. \LTY\ provides a two-phase cross-entropy optimization algorithm. 
It can quickly obtain a feasible solution while ensuring load balancing. The detailed co-clustering algorithm can be referred to in \S~\ref{sec:algo:cem} in the Appendix. The solution can then be applied to online speculative token shuffling and offline speculative expert grouping, which can be referred to in \S~\ref{sec:algo:cem} as well.

%\begin{figure}[t]
%\centering
%\includegraphics[width=.9\linewidth]{figures/co_shf_example_v2.pdf}
%\caption{Example of token-expert conjugacy scheduling}
%\label{fig:co_shf_example}
%\end{figure}



==> motivation.tex <==
\section{Empirical Study of Token-expert Affinity}\label{sec:bkg}

% \subsection{Reducing communication overhead of DS-MoE}\label{sec:bkg:moe}

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{figures/ds-moe-vs-s-moe.pdf}
%     \caption{DS-MoE v.s. s-MoE when DP $\ge$ 2.}
%     \label{fig:dp-ep-tp}
% \end{figure}

\subsection {Intra-layer bi-clustered token-expert Conjugacy}\label{sec:bkg:token-expert}
Within each MoE layer, each expert module in an LLM layer is trained to process a particular semantic domain of tokens. Tokens and experts exhibit high affinity in different dimensions. We profile the intermediate activation of the gating module in each MoE layer in the DeepSeek-MoE-16B and Mixtral-8x7B. One important observation shows that strong bi-clustered conjugacy between tokens and experts, as shown in Figure~\ref{fig:4d_affinity_example}. That is, experts are likely to be activated by a certain sub-group of tokens with high semantic affinity, while are not likely to be activated by other general tokens in vocabulary. And from tokens perspective, it is true that semantically similar tokens are likely to activate a certain sub-group of experts. We name this phenomenon bi-clustered conjugacy.

\paragraph{Inter-layer expert-expert affinity} The left picture of Figure~\ref{fig:inter_layer_example} shows the activation correlation of the 4th and 5th layer of the Mixtral-8x7B model. The x-/y-axis represents the expert groups of a layer. For Mixtral-8x7B, each token is routed 2 out of 8 experts at each layer. Thus, the number of expert groups at each layer is ${8 \choose 2}=28$. When tokens choose some concrete experts at the fourth layer, they tend to choose a rather fixed set of experts at the next layer with high probability. We name this phenomenon \textit{inter-layer expert-expert affinity}.

\begin{figure}[t!]
    \centering
    \subfigure[Example of intra-layer token-expert activation map (1st MoE layer of DeepSeek-MoE-16B profiled using the LongBench dataset). Darker color in the map indicates higher activation frequency or stronger correlation.]{
    \label{fig:intra_layer_example}
    \includegraphics[width=.5\linewidth]{figures/intra-layer-affinity.pdf}
    }
    \subfigure[Example of inter-layer expert-expert correlation map (4th/5th MoE layer of Mixtral-8x7B profiled using the LongBench dataset). Darker color in the map indicates stronger correlation.]{
    \label{fig:inter_layer_example}
    \includegraphics[width=.5\linewidth]{figures/inter-layer-affinity.pdf}
    }
    \subfigure[Example of perfromance of \texttt{allreduce} and \texttt{all2all} under different local activation ratio ($\alpha$).]{
    \label{fig:ar_vs_a2a}
    \includegraphics[width=.5\linewidth]{figures/ar-vs-a2a.pdf}
    }
    \caption{Conjugacy illustration and collective communication micro-benchmark.}
    % \vspace{-0.5cm}
    \label{fig:4d_affinity_example}
\end{figure}

\paragraph{Simple conditional probability model for token activation path}
The above examples illustrate the tabularized relationship between tokens and experts. We argue that, simple conditional probability model can work to predict the activation path of tokens by combining the above intra-layer conjugacy and/inter-layer affinity.
We first calculate the kurtosis\footnote{Kurtosis is a measure of the tailedness of a distribution. High Kurtosis indicates a token favors several fixed experts during multiple occurrences.} of each token's activation map. The right picture of Figure~\ref{fig:intra_layer_example} shows most of the kurtosis values are higher than 8, indicating that the to-route experts for each token concentrate on a narrowed set, regardless of the context. We further use partial (25\%) of the profile dataset to calculate each tokens' most routed top-k experts. Then the static top-k experts are used to predict the tokens activation using the left part (75\%) of the profile dataset, achieving a 96.3\% precision and a 78.8\% F1 score. The right part of Figure~\ref{fig:inter_layer_example} predicts the next-layer-activation via looking back the prior layers. As we know more about the previous activation sequence at layer $L$, we can predict the activation at layer $L + 1$ with higher confidence (about 70\% when looking back 5 layers).

\paragraph{Expert pre-grouping and token re-batching}
Leveraging the intrinsic conjugacy between tokens and experts in MoE models to achieve token-expert co-dispatching, may help reduce communication volume and boost distributed parallel inference. First, similar experts can be pre-grouped together at deployment time based on pre-profiled and modeled affinity. Second, on the fly, individual tokens can be re-shuffled and re-batched to the GPU devices that host the expert groups whose member experts have largest modeled conjugacy with the token. Such co-scheduling aims to avoid scattered, cross-device token-expert activations, or equivalently, maximize the probability of intra-device, local activations. Figure~\ref{fig:ar_vs_a2a} shows an micro-benchmark experiment, testing the \texttt{all2all} latency under different local activation rate using the \textit{nccl} \texttt{all2allv} API. With the local activation rate ($\alpha$) varying from 0.2 to 0.9, the latency decreases gradually, showing the performance gains with improved expert-token co-scheduling.

\begin{algorithm}[h!]
  \small
      \DontPrintSemicolon
      \caption{CEO-based co-clustering algorithm}
      \label{algo:cem}
      
      \SetKwFunction{FMIN}{min}
      \SetKwFunction{FOnes}{ones}
      \SetKwFunction{FSum}{sum}
      \SetKwFunction{FNorm}{norm}
      \SetKwFunction{FSample}{sample}
      \SetKwFunction{FLen}{len}
      \SetKwFunction{FArgmax}{argmax}
      \SetKwFunction{FIdmax}{argmax\_with\_values}

      \SetKwInput{Input}{input}\SetKwInput{Output}{output}
      
      \Input{$n\_steps$: number of iteration steps; $T$: token-expert activation matrix; $K$: number of samples of each sampling; $N$: number of experts per layer; $E$: number of co-clusters; $t$: number of tokens; $f$: token load-balance factor; $\rho$: percentage of tokens to choose during each iteration}
      \Output{$\mathcal{E}$: expert labels; $\mathcal{T}$: token labels; $\mathcal{T}_p$: confidence of tokens choosing specific experts}
      
      \SetKwProg{Fn}{Function}{:}{}
      
      $p\_matrix\_ep$ $\gets$ \FOnes{$N$, $E$} $/$ $E$
      
      $p\_matrix\_tk$ $\gets$ \FOnes{$t$, $E$} $/$ $E$

      \Fn{\FSample{$p\_matrix$, $n\_samples$, $type$, $\beta$}}{
          $samples$ $\gets$ empty list
          
          \Repeat{generated $n\_samples$ samples}{
              $mask$ $\gets$ \FOnes{$E$}
              
              $cnter$ $\gets$ hash map (default value is 0)
              
              $sample$ $\gets$ empty list
              
              \For{$i$ from $0$ to \FLen{$p\_matrix$}$ - 1$}{
                  $p$ $\gets$ \FNorm{$p\_matrix[i] * mask$}
                  
                  $cls$ $\gets$ sample a value from a multinomial distribution with $p$
                  
                  \If{$type$ is $expert$}{
                      $cnter[cls]$ $\gets$ $cnter[cls] + 1$
                      
                      \If{$cnter[cls]$ $==$ $E$}{
                          $mask[cls]$ $\gets$ 0
                      }
                  }
                  \If{$type$ is $token$}{
                      $cnter[cls]$ $\gets$ $cnter[cls] + $ \FSum{$T[i]$}
                      
                      \If{$cnter[cls]$ $>=$ \FSum{$T$} $/$ $E * \beta$}{
                          $mask[cls]$ $\gets$ 0
                      }
                  }
              }
              append $sample$ to $samples$
          }
          \KwRet{$samples$}
      }\;

      \Repeat{iterating for $n\_steps$ steps}{
          $ep\_samples$ $\gets$ \FSample{$p\_matrx\_ep$, $K$, $expert$}
          
          $tk\_samples$ $\gets$ \FSample{$p\_matrx\_tk$, $K$, $token$, $f$}
          
          $scores$ $\gets$ summation of $T$ of the same co-clusters
          
          $better\_samples$ $\gets$ samples with top-$\rho \times 100\%$ scores
          
          update $p\_matrix\_ep$ and $p\_matrix\_tk$
      }\;

      $\mathcal{E}$ $\gets$ \FArgmax{$p\_matrix\_ep$, axis=$1$}
      
      $\mathcal{T}$, $\mathcal{T}_p$ $\gets$ \FIdmax{$p\_matrix\_tk$, axis=$1$}\;
\end{algorithm}

\section{Algorithm for the s-TS/s-EG Solver}\label{sec:algo:cem}
The Rubinstein Cross-Entropy Optimization (CEO) algorithm is a Monte Carlo method used primarily for optimization and importance sampling. Similar to the evolutionary algorithm, the CEO sprinkles points in space according to a certain rule, obtains the error of each point, and then determines the rule of the next round of sprinkle points according to the error information. The cross entropy method is named because the objective of the method (theoretically) is to minimize the cross entropy between the data distribution obtained by random scattered points and the actual data distribution (equivalent to minimizing the KL distance), trying to make the sampling distribution (sprinkling points) the same as the real distribution.

Algorithm ~\ref{algo:cem} describes the CEO-based token-expert co-scheduling algorithm in \LTY. The algorithm models each expert/token's choice of category as a D-dimensional polynomial distribution, and the probability of polynomial distribution is determined by $p\_matrix\_ep$ and $p\_matrix\_tk$ . Under the initial conditions, the probability of selecting each class by expert/token is set to equal. In each iteration, several class label samples are first sampled according to the probability matrix (lines 25-26). The sampling function \texttt{sample} samples label points from the D-dimensional polynomial distribution (line 11) and ensures that the number of experts in each category is equal (line 12-15). A relaxation factor $\beta$ is used to ensure that the token frequency of each category is as equal as possible (lines 16-19). After the sampling is complete, the algorithm calculates the local activation frequency of each sample (line 27) as the score, and selects samples with top-$\rho \times 100\%$ scores to update the probability matrix (line 27–line 28). After completing the $n\_steps$ iteration, the algorithm takes the cluster with the highest probability for each expert/token as its cluster label (lines 32-33). The clsuter label of expert/token actually represents the number of the device to which expert/token is scheduled. At the same time, the value of the probability matrix is used as the confidence that each token belongs to its cluster. In practice, the hyperparameters $\beta$ and $\rho$ are set as 1.1 and 0.2. By now, the token-device scheduling table $\mathcal{T}$, token-device scheduling confidence table $\mathcal{T}_p$, and expert-device scheduling table $\mathcal{E}$ are generated. After the scheduling table $\mathcal{E}$ is constructed, the experts at each layer need to be rearranged according to the scheduling table during online inference service deployment. In addition, the \LTY\ rearranges the gating module by column to implement transparent expert shuffle. The semantics of other layers are not affected. The rearranged experts are highly boxed, so that the token activation at each layer is de-cohesive, and the redundant network communication overhead caused by dispersive activation is reduced.

\subsection{Modeling Inter-layer Activation Conjugacy}
Leveraging the conditional probability model described in \S~\ref{sec:bkg:token-expert}, we use a simple probability-based first-order Marcov chain to model the inter-layer activation conjugacy. To reduce the combination space, we model the activation device sequence rather than the activation expert sequence, because we only care about the device-level token rebatching. When looking back $l$ layers, we construct a table shaped like $[E^l, E]$, where the row of the table indicates the sequence of devices selected at the previous $l$ layers and the column indicates the probability of activating the $E$ devices in the current layer. Like the \S~\ref{sec:algo:cem} shows, we also calculate the activation sequence to device table $\mathcal{A}$ and the confidence table $\mathcal{A}_p$. In practice, we set the number of looking-back layers as 2.

\subsection{Speculative Token Shuffling on the Fly Based on Fast Lookup}

To reduce the combination space, we model the activation device
sequence rather than the activation expert sequence, because we only care about the device-level token rebatching.

% \section{Detailed Online Re-rebatching Algorithm}

We implement a fast online re-batching mechanism based on fast looking-up tables (Algorithm~\ref{algo:fast_shf}). The algorithm queries the token-device scheduling table $\mathcal{T}$ and activation-sequence-device table $\mathcal{S}$, together with their confidences first. Then, the table with higher confidence is adopted to obtain the device ID list to which the current batch token needs to be shuffle (line 2). The algorithm performs the argsort operation to obtain the shuffle indicators (line 3) of the token. Then, the final shuffle indicators are obtained by grouping, aligning, and concatenation, and the token is shuffled (line 4 to line 7). After rebatching is complete, \LTY\ calls the \texttt{reduce-scatter} operation. After MoE computing is complete, \LTY\ runs the \texttt{allgather} operation to collect tokens. Finally, the order of tokens are shuffled back based on the previously calculated shuffle indicators (lines 14-18). The entire \texttt{rebatch} and \texttt{resume} processes do not involve load calculation and decision-making. They are directly completed by querying tables. The runtime overhead mainly involves large token matrix shuffling, which we optimize via high-performance kernels. The memory occupation of the scheduling tables is negligible. For example, for DeepSeek-V2, the memory space that the token-to-device table $\mathcal{T}$ occupies is $\frac{102400 \times 60 \times 2}{1024^2} \approx 11.72 MB$ (assuming the data format is \texttt{int16}).

\begin{algorithm}[t]
  \small
  \DontPrintSemicolon
  \caption{Online re-batching based on fast lookup}
  \label{algo:fast_shf}
  
  \SetKwFunction{FSHF}{rebatch\_tokens}
  \SetKwFunction{FRES}{resume\_tokens}
  \SetKwFunction{FASORT}{argsort}
  \SetKwFunction{FALIGN}{align}
  \SetKwFunction{FGBK}{group\_by\_key}
  \SetKwFunction{FCAT}{concat}
  \SetKwFunction{FRS}{reduce\_scatter}
  \SetKwFunction{FAG}{allgather}
  \SetKwFunction{FCOND}{cond}
  
  \SetKwInput{Input}{input}\SetKwInput{Output}{output}
  
  \Input{$\mathcal{B} \in \mathbb{N}^{n}$: Input token IDs; $\mathcal{T}$: token-device Schedule Table}
  
  \SetKwProg{Fn}{Function}{:}{}
  
      \Fn{\FSHF{$\mathcal{B},\mathcal{T}$}}{
          % $dev\_ids\_T$ $\gets$ $\mathcal{T}\left[\mathcal{B}\right]$\;
          % $dev\_ids\_A$ $\gets$ $\mathcal{A}\left[\mathcal{B}\right]$\;
          $dev\_ids$ $\gets$ \FCOND{$\mathcal{T}_p\left[\mathcal{B}\right] > \mathcal{A}_p\left[\mathcal{B}\right]$, $\mathcal{T}\left[\mathcal{B}\right]$, $\mathcal{A}\left[\mathcal{B}\right]$}
          
          % \tcp*[l]{sort token IDs according to device IDs}
          $shf\_indices$ $\gets$ \FASORT{$dev\_ids$}
          
  
          % \tcp*[l]{group tokens according to device IDs}
          $g\_shf\_indices$ $\gets$ \FGBK{$shf\_indices$}
          
          % \tcp*[l]{align bins by round-robin picking-packing}
          $g\_shf\_indices$ $\gets$ \FALIGN{$g\_shf\_indices$}
          
          % \tcp*[l]{get the shuffle indices via concatting}
          $shf\_indices$ $\gets$ \FCAT{$g\_shf\_indices$}
          
          $\mathcal{B}$ $\gets$ $\mathcal{B}\left[shf\_indices\right]$
          
          \KwRet{$shf\_indices$}
      } \;
  
      \Fn{\FRES{$\mathcal{B},shf\_indices$}}{
          $r\_shf\_indices$ $\gets$ \FASORT{$shf\_indices$}
          
          $\mathcal{B}$ $\gets$ $\mathcal{B}\left[r\_shf\_indices\right]$
      } \;
  
      $shf\_indices$ $\gets$ \FSHF{$\mathcal{B},\mathcal{T}$}
      
      $\mathcal{B}_{local}$ $\gets$ \FRS{$\mathcal{B}$}
      
      executing MoE layer
      $\mathcal{B}$ $\gets$ \FAG{$\mathcal{B}_{local}$}
      
      \FRES{$\mathcal{B}$,$shf\_indices$}
  \end{algorithm}



==> motivation_2.tex <==
\section{Empirical Study of Token-expert Affinity}\label{sec:bkg}

% \subsection{Reducing communication overhead of DS-MoE}\label{sec:bkg:moe}

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{figures/ds-moe-vs-s-moe.pdf}
%     \caption{DS-MoE v.s. s-MoE when DP $\ge$ 2.}
%     \label{fig:dp-ep-tp}
% \end{figure}

\subsection {Intra-layer bi-clustered token-expert Conjugacy}\label{sec:bkg:token-expert}
Within each MoE layer, each expert module in an LLM layer is trained to process a particular semantic domain of tokens. Tokens and experts exhibit high affinity in different dimensions. We profile the intermediate activation of the gating module in each MoE layer in the DeepSeek-MoE-16B and Mixtral-8x7B. One important observation shows that strong bi-clustered conjugacy between tokens and experts, as shown in Figure~\ref{fig:4d_affinity_example}. That is, experts are likely to be activated by a certain sub-group of tokens with high semantic affinity, while are not likely to be activated by other general tokens in vocabulary. And from tokens perspective, it is true that semantically similar tokens are likely to activate a certain sub-group of experts. We name this phenomenon bi-clustered conjugacy.

\paragraph{Inter-layer expert-expert affinity} The left picture of Figure~\ref{fig:inter_layer_example} shows the activation correlation of the 4th and 5th layer of the Mixtral-8x7B model. The x-/y-axis represents the expert groups of a layer. For Mixtral-8x7B, each token is routed 2 out of 8 experts at each layer. Thus, the number of expert groups at each layer is ${8 \choose 2}=28$. When tokens choose some concrete experts at the fourth layer, they tend to choose a rather fixed set of experts at the next layer with high probability. We name this phenomenon \textit{inter-layer expert-expert affinity}.

\begin{figure}[t!]
    \centering
    \subfigure[Example of intra-layer token-expert activation map (1st MoE layer of DeepSeek-MoE-16B profiled using the LongBench dataset). Darker color in the map indicates higher activation frequency or stronger correlation.]{
    \label{fig:intra_layer_example}
    \includegraphics[width=.5\linewidth]{figures/intra-layer-affinity.pdf}
    }
    \subfigure[Example of inter-layer expert-expert correlation map (4th/5th MoE layer of Mixtral-8x7B profiled using the LongBench dataset). Darker color in the map indicates stronger correlation.]{
    \label{fig:inter_layer_example}
    \includegraphics[width=.5\linewidth]{figures/inter-layer-affinity.pdf}
    }
    \subfigure[Example of perfromance of \texttt{allreduce} and \texttt{all2all} under different local activation ratio ($\alpha$).]{
    \label{fig:ar_vs_a2a}
    \includegraphics[width=.5\linewidth]{figures/ar-vs-a2a.pdf}
    }
    \caption{Conjugacy illustration and collective communication micro-benchmark.}
    % \vspace{-0.5cm}
    \label{fig:4d_affinity_example}
\end{figure}

\paragraph{Simple conditional probability model for token activation path}
The above examples illustrate the tabularized relationship between tokens and experts. We argue that, simple conditional probability model can work to predict the activation path of tokens by combining the above intra-layer conjugacy and/inter-layer affinity.
We first calculate the kurtosis\footnote{Kurtosis is a measure of the tailedness of a distribution. High Kurtosis indicates a token favors several fixed experts during multiple occurrences.} of each token's activation map. The right picture of Figure~\ref{fig:intra_layer_example} shows most of the kurtosis values are higher than 8, indicating that the to-route experts for each token concentrate on a narrowed set, regardless of the context. We further use partial (25\%) of the profile dataset to calculate each tokens' most routed top-k experts. Then the static top-k experts are used to predict the tokens activation using the left part (75\%) of the profile dataset, achieving a 96.3\% precision and a 78.8\% F1 score. The right part of Figure~\ref{fig:inter_layer_example} predicts the next-layer-activation via looking back the prior layers. As we know more about the previous activation sequence at layer $L$, we can predict the activation at layer $L + 1$ with higher confidence (about 70\% when looking back 5 layers).

\paragraph{Expert pre-grouping and token re-batching}
Leveraging the intrinsic conjugacy between tokens and experts in MoE models to achieve token-expert co-dispatching, may help reduce communication volume and boost distributed parallel inference. First, similar experts can be pre-grouped together at deployment time based on pre-profiled and modeled affinity. Second, on the fly, individual tokens can be re-shuffled and re-batched to the GPU devices that host the expert groups whose member experts have largest modeled conjugacy with the token. Such co-scheduling aims to avoid scattered, cross-device token-expert activations, or equivalently, maximize the probability of intra-device, local activations. Figure~\ref{fig:ar_vs_a2a} shows an micro-benchmark experiment, testing the \texttt{all2all} latency under different local activation rate using the \textit{nccl} \texttt{all2allv} API. With the local activation rate ($\alpha$) varying from 0.2 to 0.9, the latency decreases gradually, showing the performance gains with improved expert-token co-scheduling.

\begin{algorithm}[h!]
  \small
      \DontPrintSemicolon
      \caption{CEO-based co-clustering algorithm}
      \label{algo:cem}
      
      \SetKwFunction{FMIN}{min}
      \SetKwFunction{FOnes}{ones}
      \SetKwFunction{FZeros}{zeros}
      \SetKwFunction{FSum}{sum}
      \SetKwFunction{FNorm}{norm}
      \SetKwFunction{FSample}{sample}
      \SetKwFunction{FLen}{len}
      \SetKwFunction{FArgmax}{argmax}
      \SetKwFunction{FIdmax}{argmax\_with\_values}

      \SetKwInput{Input}{input}\SetKwInput{Output}{output}
      
      \Input{$n\_steps$: number of iteration steps; \\ $\bm{\mathcal{C}}_p$: the token-2-expert confidence table; $\bm{a}$: the token frequency; \\ $K$: number of samples of each sampling; $N$: number of experts per layer; \\ $E$: number of co-clusters; $t$: number of tokens; \\ $f$: token load-balance factor; \\ $\rho$: percentage of tokens to choose during each iteration}
      \Output{$\mathcal{E}$: expert labels; $\mathcal{T}$: token labels; \\ $\mathcal{T}_p$: confidence of tokens choosing specific experts}
      
      \SetKwProg{Fn}{Function}{:}{}
      
      $p\_matrix\_ep$ $\gets$ \FOnes{$N$, $E$} $/$ $E$
      
      $p\_matrix\_tk$ $\gets$ \FOnes{$t$, $E$} $/$ $E$

      \Fn{\FSample{$p\_matrix$, $n\_samples$, $type$, $\beta$}}{
          $samples$ $\gets$ empty list
          
          \Repeat{generated $n\_samples$ samples}{
              $mask$ $\gets$ \FOnes{$E$}
              
              $cnter$ $\gets$ \FZeros{$E$}, hash map (default value is 0)
              
              $sample$ $\gets$ empty list
              
              \For{$i$ from $0$ to \FLen{$p\_matrix$}$ - 1$}{
                  $p$ $\gets$ \FNorm{$p\_matrix[i] * mask$}
                  
                  $cls$ $\gets$ sample a value from a multinomial$(1,E,p)$
                  
                  \If{$type$ is $expert$}{
                      $cnter[cls]$ $\gets$ $cnter[cls] + 1$
                      
                      \If{$cnter[cls]$ $==$ $N/E$}{
                          $mask[cls]$ $\gets$ 0
                      }
                  }
                  \If{$type$ is $token$}{
                      $cnter[cls]$ $\gets$ $cnter[cls] + $ \FSum{$\bm{\mathcal{C}}_p[i]*\bm{a}[i]$}
                      
                      \If{$cnter[cls]$ $>=$ \FSum{$\bm{\mathcal{C}}_p*\bm{a}$} $/$ $E * \beta$}{
                          $mask[cls]$ $\gets$ 0
                      }
                  }
                  append $cls$ to $sample$
              }
              append $sample$ to $samples$
          }
          \KwRet{$samples$}
      }\;

      \Repeat{iterating for $n\_steps$ steps}{
          $ep\_samples$ $\gets$ \FSample{$p\_matrx\_ep$, $K$, $expert$}
          
          $tk\_samples$ $\gets$ \FSample{$p\_matrx\_tk$, $K$, $token$, $f$}
          
          $scores$ $\gets$ summation of $T$ of the same co-clusters
          
          $better\_samples$ $\gets$ samples with top-$\rho \times 100\%$ scores
          
          update $p\_matrix\_ep$ and $p\_matrix\_tk$
      }\;

      $\mathcal{E}$ $\gets$ \FArgmax{$p\_matrix\_ep$, axis=$1$}
      
      $\mathcal{T}$, $\mathcal{T}_p$ $\gets$ \FIdmax{$p\_matrix\_tk$, axis=$1$}\;
\end{algorithm}

\section{Algorithm for the s-TS/s-EG Solver}\label{sec:algo:cem}
The Rubinstein Cross-Entropy Optimization (CEO) algorithm is a Monte Carlo method used primarily for optimization and importance sampling. Similar to the evolutionary algorithm, the CEO sprinkles points in space according to a certain rule, obtains the error of each point, and then determines the rule of the next round of sprinkle points according to the error information. The cross entropy method is named because the objective of the method (theoretically) is to minimize the cross entropy between the data distribution obtained by random scattered points and the actual data distribution (equivalent to minimizing the KL distance), trying to make the sampling distribution (sprinkling points) the same as the real distribution.

Algorithm ~\ref{algo:cem} describes the CEO-based token-expert co-scheduling algorithm in \LTY. The algorithm models each expert/token's choice of category as a D-dimensional multinomial distribution, and the probability of polynomial distribution is determined by $p\_matrix\_ep$ and $p\_matrix\_tk$ . Under the initial conditions, the probability of selecting each class by expert/token is set to equal. In each iteration, several class label samples are first sampled according to the probability matrix (lines 25-26). The sampling function \texttt{sample} samples label points from the D-dimensional polynomial distribution (line 11) and ensures that the number of experts in each category is equal (line 12-15). A relaxation factor $\beta$ is used to ensure that the token frequency of each category is as equal as possible (lines 16-19). After the sampling is complete, the algorithm calculates the local activation frequency of each sample (line 27) as the score, and selects samples with top-$\rho \times 100\%$ scores to update the probability matrix (line 27–line 28). After completing the $n\_steps$ iteration, the algorithm takes the cluster with the highest probability for each expert/token as its cluster label (lines 32-33). The clsuter label of expert/token actually represents the number of the device to which expert/token is scheduled. At the same time, the value of the probability matrix is used as the confidence that each token belongs to its cluster. In practice, the hyperparameters $\beta$ and $\rho$ are set as 1.1 and 0.2. By now, the token-device scheduling table $\mathcal{T}$, token-device scheduling confidence table $\mathcal{T}_p$, and expert-device scheduling table $\mathcal{E}$ are generated. After the scheduling table $\mathcal{E}$ is constructed, the experts at each layer need to be rearranged according to the scheduling table during online inference service deployment. In addition, the \LTY\ rearranges the gating module by column to implement transparent expert shuffle. The semantics of other layers are not affected. The rearranged experts are highly boxed, so that the token activation at each layer is de-cohesive, and the redundant network communication overhead caused by dispersive activation is reduced.

\subsection{Modeling Inter-layer Activation Conjugacy}
Leveraging the conditional probability model described in \S~\ref{sec:bkg:token-expert}, we use a simple probability-based first-order Marcov chain to model the inter-layer activation conjugacy. To reduce the combination space, we model the activation device sequence rather than the activation expert sequence, because we only care about the device-level token rebatching. When looking back $l$ layers, we construct a table shaped like $[E^l, E]$, where the row of the table indicates the sequence of devices selected at the previous $l$ layers and the column indicates the probability of activating the $E$ devices in the current layer. Like the \S~\ref{sec:algo:cem} shows, we also calculate the activation sequence to device table $\mathcal{A}$ and the confidence table $\mathcal{A}_p$. In practice, we set the number of looking-back layers as 2.

\subsection{Speculative Token Shuffling on the Fly Based on Fast Lookup}

To reduce the combination space, we model the activation device
sequence rather than the activation expert sequence, because we only care about the device-level token rebatching.

% \section{Detailed Online Re-rebatching Algorithm}

We implement a fast online re-batching mechanism based on fast looking-up tables (Algorithm~\ref{algo:fast_shf}). The algorithm queries the token-to-expert-cluster scheduling table $\mathcal{T}$ and expert-cluster-sequence-to-expert-cluster table $\mathcal{S}$, together with their confidences first. Then, the table with higher confidence is adopted to obtain the device ID list to which the current batch token needs to be shuffle (line 2). The algorithm performs the argsort operation to obtain the shuffle indicators (line 3) of the token. Then, the final shuffle indicators are obtained by grouping, aligning, and concatenation, and the token is shuffled (line 4 to line 7). After rebatching is complete, \LTY\ calls the \texttt{reduce-scatter} operation. After MoE computing is complete, \LTY\ runs the \texttt{allgather} operation to collect tokens. Finally, the order of tokens are shuffled back based on the previously calculated shuffle indicators (lines 14-18). The entire \texttt{rebatch} and \texttt{resume} processes do not involve load calculation and decision-making. They are directly completed by querying tables. The runtime overhead mainly involves large token matrix shuffling, which we optimize via high-performance kernels. The memory occupation of the scheduling tables is negligible. For example, for DeepSeek-V2, the memory space that the token-to-device table $\mathcal{T}$ occupies is $\frac{102400 \times 60 \times 2}{1024^2} \approx 11.72 MB$ (assuming the data format is \texttt{int16}).

\begin{algorithm}[t]
  \small
  \DontPrintSemicolon
  \caption{Online re-batching based on fast lookup}
  \label{algo:fast_shf}
  
  \SetKwFunction{FSHF}{rebatch\_tokens}
  \SetKwFunction{FRES}{resume\_tokens}
  \SetKwFunction{FASORT}{argsort}
  \SetKwFunction{FALIGN}{align}
  \SetKwFunction{FGBK}{group\_by\_key}
  \SetKwFunction{FCAT}{concat}
  \SetKwFunction{FRS}{reduce\_scatter}
  \SetKwFunction{FAG}{allgather}
  \SetKwFunction{FCOND}{cond}
  
  \SetKwInput{Input}{input}\SetKwInput{Output}{output}
  
  \Input{$\mathcal{B} \in \mathbb{N}^{n}$: Input token IDs; $\mathcal{T}$: token-to-expert-cluster Schedule Table; \\ $\mathcal{A}$: expert-cluster-sequence-to-expert-cluster Schedule Table} 
  
  \SetKwProg{Fn}{Function}{:}{}
  
      \Fn{\FSHF{$\mathcal{B},\mathcal{T}$}}{
          % $dev\_ids\_T$ $\gets$ $\mathcal{T}\left[\mathcal{B}\right]$\;
          % $dev\_ids\_A$ $\gets$ $\mathcal{A}\left[\mathcal{B}\right]$\;
          $dev\_ids$ $\gets$ \FCOND{$\mathcal{T}_p\left[\mathcal{B}\right] > \mathcal{A}_p\left[\mathcal{B}\right]$, $\mathcal{T}\left[\mathcal{B}\right]$, $\mathcal{A}\left[\mathcal{B}\right]$}
          
          % \tcp*[l]{sort token IDs according to device IDs}
          $shf\_indices$ $\gets$ \FASORT{$dev\_ids$}
  
          % \tcp*[l]{group tokens according to device IDs}
          $g\_shf\_indices$ $\gets$ \FGBK{$shf\_indices$}
          
          % \tcp*[l]{align bins by round-robin picking-packing}
          $g\_shf\_indices$ $\gets$ \FALIGN{$g\_shf\_indices$}
          
          % \tcp*[l]{get the shuffle indices via concatting}
          $shf\_indices$ $\gets$ \FCAT{$g\_shf\_indices$}
          
          $\mathcal{B}$ $\gets$ $\mathcal{B}\left[shf\_indices\right]$
          
          \KwRet{$shf\_indices$}
      } \;
  
      \Fn{\FRES{$\mathcal{B},shf\_indices$}}{
          $r\_shf\_indices$ $\gets$ \FASORT{$shf\_indices$}
          
          $\mathcal{B}$ $\gets$ $\mathcal{B}\left[r\_shf\_indices\right]$
      } \;
  
      $shf\_indices$ $\gets$ \FSHF{$\mathcal{B},\mathcal{T}$}
      
      $\mathcal{B}_{local}$ $\gets$ \FRS{$\mathcal{B}$}
      
      executing MoE layer
      
      $\mathcal{B}$ $\gets$ \FAG{$\mathcal{B}_{local}$}
      
      \FRES{$\mathcal{B}$,$shf\_indices$}
  \end{algorithm}


